A Probabilistic Model of Activity Recognition with Loose Clothing

Human activity recognition has become an attractive research area with the development of on-body wearable sensing technology. With comfortable electronic-textiles, sensors can be embedded into clothing so that it is possible to record human movement outside the laboratory for long periods. However, a long-standing issue is how to deal with motion artefacts introduced by movement of clothing with respect to the body. Surprisingly, recent empirical findings suggest that cloth-attached sensor can actually achieve higher accuracy of activity recognition than rigid-attached sensor, particularly when predicting from short time-windows. In this work, a probabilistic model is introduced in which this improved accuracy and resposiveness is explained by the increased statistical distance between movements recorded via fabric sensing. The predictions of the model are verified in simulated and real human motion capture experiments, where it is evident that this counterintuitive effect is closely captured.

==> background.tex <==
%\mh{\sref{background} needs to be linked to the preceding section. Give a more specific and in-depth discussion of the issue you are addressing, and why it's important. State the ways that others have approached it. Explain your approach, and why it is a contribution beyond the state of the art.}

%\subsection{Mutual information}\label{s:mutual_information}
%\mh{\sref{mutual_information} needs to be connected to the rest of the paper. As a reader, it is unclear why you are suddenly discussing \gls{mi}.}
%\Gls{mi} is an approach to tell the degree of difficulty to know the variable from the other variable, it also can be thought as the reduction of uncertainty of knowing about one variable, when another is given \cite{cover_elements_2012}.\mh{Rephrase.}\id{I think that I know what you mean, but I suggest to clarify these initial sentences}

%Formally, the \acrlong{mi} for two variables $X$ and $Y$ is given as \cite{cover_elements_2012}\edit{.}{}{mh} 
%\begin{equation}
%I(X;Y) = H(X)+H(Y)-H(X,Y)
%\label{mi}
%\end{equation}
%\mh{Symbols that have not been defined or explained: $X,Y,\mathcal{Y},\mathcal{X}$.}
%where $H(X)$, $H(Y)$ denote the entropy of $X$ and $Y$, and $H(X,Y)$  is their joint entropy. The calculation of entropy and joint entropy are shown in equation \eqref{entropy} and equation \eqref{joint_entropy}.
%\mh{What is the intuitive meaning of \eref{mi}? Can you explain why it takes this form?}

%\begin{equation}
%H(X)=-\sum_{i=1}^{n}P(X_{i})log_{2}P{(X_{i}})
%\label{entropy}
%\end{equation}

%\begin{equation}
%H(X,Y)=-\sum_{i=1}^{n}\sum_{j=1}^{n}P(X_{i},Y_{j})log_{2}[P(X_{i},Y_{j})]
%\label{joint_entropy}
%\end{equation}
%Where $P(X)$, $P(Y)$ denote the marginal probabilities of $X$ and $Y$, and $P(X,Y)$ denotes the joint probability.

%This concept can be used in classification and regression.\mh{From here...} \edit{Activity recognition}{\Gls{ar}}{mh} (\edit{}{\ie}{mh} classification) aims to automatically classify movements into a number of activities (\eg running, walking) when class data is provided. The more reduced uncertainty of label prediction means better classification performance while less reduced uncertainty shows worse classification accuracy. 

%In \edit{motion estimation}{\gls{me}}{mh} (\edit{}{\ie}{mh} regression), human motion measurement (\eg gait kinematics, walking/running speed) can be seen as label, in experiments, actual human motion is collected from body-attached sensor due to they are rigidly attached while cloth-attached sensor measurement contains motion artifacts so it uses cloth-attached sensor measurement to regress body-attached sensor measurement. Low mutual information tells that it is challenge to predict human motion when cloth-attached sensors measurement is known while high mutual information shows it is simple to notice human motion from cloth-attached sensors measurement. 
%\mh{... to here has nothing to do with \gls{mi}: it is a discussion about behaviour analysis.} \id{this whole section is extremely confusing. I think that you need to limit the explanation of the theory that is well established and focus more on your specific application}

%Therefore, a hypothesis that mutual information should be positively corresponding to classification accuracy and inversely proportional with mean squared error in regression is proposed.\mh{If this is the main way to measure the use of the \gls{mi}, then showing this correlation for several different classification and regression approaches would strengthen your argument.}

%Correlation coefficient (\eg\gls{pcc}) is anther method to find the relationship between two variables.\mh{It is unclear why you include this paragraph. Will you use this?} The main difference with \gls{mi} measures the general dependence while \gls{pcc} only can measure the linear dependence. \cite{clavier_mutual_2009}\mh{Broken reference.} Therefore, \gls{pcc} is not well suited to the task of human motion analysis. The reason is there is no linear relationship between class data and class label (see Fig.~\ref{re}(A)). Moreover, \gls{mi} is a more general method, more widely to be used and it can handle more complicated data or situation. But, the advantage of \gls{pcc} is simpler and more sufficient \cite{li_mutual_1990}.\mh{Broken reference.} 
%\mh{\done{What other measures could you use? Why do you choose \gls{mi} instead of those measures?}}
%\mh{Did you take a look at \textcite{Reshef2011}?}
%\mh{\done{The preceding two paragraphs need rewriting to make them clearer. It would be better to describe in general terms first, then go to the specific problems your paper considers. For instance, ``\Gls{mi} quantifies how much knowing one random variable (\eg $X$) tells us about the other (\eg $Y$) --see, \eg \textcite{murphy_machine_2012}. In the cases considered here, the random variables represent the sensor reading and the quantity of interest (activity in classification, or motion feature in regression).''}}
%\mh{The whole of \sref{background} needs rewriting to make it clearer. The text should follow a logical sequence, gradually building up your arguments. At the moment, this section reads like a random collection of ideas, but it is not clear what ties everything together. I suggest describing the problem in general terms first, then going into the specifics.}

\subsection{Entropy}\label{s:entropy}
The entropy of a random variable is the average level of uncertainty inherent in the variable's possible outcomes. Considering the event $q$ with possible outcomes $q_{1},...q_{n}$ with possibility of $P(q_{1}),...P(q_{n})$, the entropy of event $q$ can be computed as \eqref{entropy}.

\begin{equation}
H(q)=-\sum_{i=1}^{n}P(q_{i})log_{2}P{(q_{i}})
\label{entropy}
\end{equation}


%\begin{equation}
%H(x_{i}) = -\sum_{i=1}^{n}\sum_{i=1}^{i} \alpha_i\frac{1}{\sqrt{|\Sigma_i|(2\pi)^d}}\exp(-\frac{1}{2}(x-\mu_i)\Sigma^{-1}(x-\mu_i)\top)\log_{2}{\alpha_i\frac{1}{\sqrt{|\Sigma_i|(2\pi)^d}}\exp(-\frac{1}{2}(x-\mu_i)\Sigma^{-1}(x-\mu_i)\top)}
%\label{entropy_gmm}
%\end{equation}


\subsection{\gls{em} algorithm for \gls{gmm}}\label{s:em}

\gls{gmm} consists of several Gaussian distributions. The Gaussian density can be expressed by equation \eqref{gmm} \cite{lan2006estimating}.
\begin{equation}
p(x) = \sum_{i=1}^{i} \omega G_i(x)
\label{gmm}
\end{equation}
Where $G_i(x)$ is the \gls{pdf} of each Gaussian component, $\omega_m$ is the weights for the corresponding component, $\sum_{i=1}^{i} \omega_i =1$ and $i$ is the number of single Gaussian in \gls{gmm}.

\gls{em} algorithm is an iteration method to maximum likelihood estimation, which is used to estimate parameters of Gaussian distribution and split \gls{gmm} in this paper \cite{mclachlan2004algorithm}.

\subsection{Entropy of the \gls{gmm}}\label{s:entropy_gmm}
The \gls{pdf} of multivariate Gaussian distribution is know as equation \eqref{pdf}.

\begin{equation}
p(x|\mu,\Sigma) = \frac{1}{\sqrt{|\Sigma|(2\pi)^d}}\exp(-\frac{1}{2}(x-\mu)\Sigma^{-1}(x-\mu)\top)
\label{pdf} 
\end{equation}
Referring from equation \eqref{entropy} \eqref{gmm} and \eqref{pdf}, the entropy of \gls{gmm} can be computed.


\subsection{\gls{js}}\label{s:js}
\gls{js} measures the similarity of two probability distributions ($p$ and $q$). Based on a variant of \gls{kl}, it solves the problem of asymmetry of \gls{kl}. Generally, the \gls{js} is symmetric, and its value is between $0$ and $1$. It is defined as equation \eqref{js}.
\begin{equation}
JS(p:q) = H(\frac{p+q}{2}) - \frac{H(p)+H(q)}{2}
\label{js} 
\end{equation}

The JS divergence is zero only if \gls{pdf} $p$ and $q$ are completely the same. While it gets one when they are completely different.  


\subsection{KS test}\label{s:ks}
Data shifting represents train data and test data are different. It is obviously found in the fabric motion because its movement generates non-stationary environment. KS test is used to to analyze whether two data distributions have a significant different based on cumulative distribution function.


\subsection{Support vector machine}\label{s:support_vector_machine}
Support vector machine (\gls{svm}) is one of supervised machine learning algorithms \cite{noble_what_2006} that is used to analyze data through classification and regression in this paper.
%\id{It is not clear what you are trying to suggest here}
%\mh{\done{Apart from \sref{support_vector_machine}, \sref{materials_and_methods} is largely background/theory \emph{not} materials and methods. I suggest you rename it to ``Background'', and rename \sref{experiments_and_material} as ``Materials and Methods''.}}

==> comments.tex <==
% define simple todo command
%\usepackage{lineno}
\usepackage[normalem]{ulem}                                        % for striking text out
\usepackage{marginnote}
\setlength{\marginparwidth}{1.75cm}
\setlength{\marginparsep}{.1mm}
\usepackage[textwidth=\marginparwidth,colorinlistoftodos]{todonotes}
\providecommand{\tinytodo}[2][]
{\todo[caption={#2}, size=\small, #1]{\renewcommand{\baselinestretch}{0.6}\selectfont#2\par}}

% define colours for to-dos
\colorlet{jb}{red}
\colorlet{mh}{red}
\providecommand{\commentcolourcode}{Comments colour code: 
{\color{mh}MH}} 
\providecommand  {\colorsout}[1]{\bgroup\markoverwith{\textcolor{#1}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon} % define coloured strike out
\providecommand{\atMH} {{\color{mh}@MH}}
\providecommand{\atJB} {{\color{jb}@JB}}

\providecommand  {\done}   [1]{\sout{#1}}
\providecommand  {\edit}   [3]{\colorsout{#3}{#1}{\color{#3}{#2}}}
\providecommand  {\nomment}[2]{\tinytodo[color=white,nolist,linecolor=#2,bordercolor=white,noinline]{\protect{\scriptsize\color{#2}#1}}}
\providecommand  {\note}[2]{\tinytodo[color=white,linecolor=#2,bordercolor=white,noinline]{\protect{\scriptsize\color{#2}#1}}}
%\providecommand  {\at}     [1]{\textcolor{#2}{@#2}}

\providecommand{\cn}{\note{Citation needed.}{mh}} % shortcut commenting commands


\providecommand{\makecomments}{%
\section*{Usage notes}~\\%[1ex]
\noindent Use \texttt{\textbackslash note\{your comment\}\{your initials\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash note\{Comment.\}\{jb\}}.\nomment{These comments will appear as margin notes. They will also appear in the todo list on the first page.}{jb} \\[2ex]
%\noindent Optionally, use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash note\{\textbackslash atJB: Please fix this.\}\{mh\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash note\{\textbackslash done\{\textbackslash atJB: Please fix this.\}\}\{mh\}}). It will then be formatted like this: \done{\atJB: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
\printacronyms~\\[2ex]% if using glossaries package to manage acronyms, print them
\listoftodos~\\[2ex]
\clearpage\setcounter{page}{1}
%\linenumbers%
}

\providecommand{\makenotes}{\clearpage\appendix\input{notes}}%

\providecommand{\makefinal}{%
\renewcommand{\makecomments}{}\renewcommand{\makenotes}{}\renewcommand{\note}[1]{}\renewcommand{\done}[1]{}\renewcommand{\edit}[3]{\#2}\renewcommand{\comment}[2]{}%
}


==> data/material_and_methods.tex <==
%\parskip 
As noted in \sref{fabric_motion_model}, the extent to which fabric motion helps \gls{ar} in practice will depend on both the \emph{complexity of the movement} and the \emph{physical properties of the fabric}. In this section, \ref{N_case_studies} empirical case studies are presented to test the model's predictions when using a well-established statistical machine learning approach for \gls{ar} with fabric-induced motion data. The cases considered are \il{\item a numerical simulation of example described in \sref{shm}\item\label{v:scotch}its physical realisation and \item\label{v:human} a real human \gls{ar} task}.

%\subsection{Material and Methods}\label{s:mnm}
\newcounter{casestudy}
\stepcounter{casestudy}%
\subsection{Case Study \thecasestudy: Simple Harmonic Motion}\label{s:sim}
%\mh{\done{For each experiment reported, this section should give a description of how the experiment is set up and conducted, at a sufficient level of detail that a competent, independent researcher could repeat it. Write it as if it were a recipe - you need to describe all the ingredients (\ie materials) needed and then the steps taken (\ie method).}}
%
%\mh{\done{Describe the aim of the experiment, and then justify the experimental design with reference to the aim.}}
%\id{the first paragraph comes out of nowhere, should you explain the idea of using a pendulum model as part of your background?}
%
This evaluation aims to verify the predictions \edit{made in \sref{shm}}{of the proposed model}{mh} using a numerical simulation. %
%a physical, instrumented mechanism to realise the experiment.
\edit{The protocol is as follows.}{}{mh}
%\mh{\done{A physical experiment would be better - let's see what comes out of your work with the scotch yoke.}}

\subsubsection{Materials and Methods}\label{s:scotch_yoke:mnm}
Data is collected from a numerical simulation of the system shown in \fref{simulation}\ref{f:simulation-a} implemented in MATLAB R2019b (MathWorks, USA) consisting of %a set of $\Nd=\NdscotchYokeSimulation$ 
trajectories of length $\Tk=\TkscotchYokeSimulation$\,\si{\second} 
generated at a sampling rate of $\fk=\SI{\fscotchYokeSimulation}{\Hz}$ using \eref{Xf} from random starting angles $\phiy \sim\U(-\pi,\pi)$ with $\Ay=\SI{\AscotchYokeSimulation}{\metre}$. %\mh{\done{How did you set the start state of the trajectories?}} 
Each data set contains $\Nd=\NdscotchYokeSimulation$ trajectories with $\NdscotchYokeSimulationLo$ trajectories from the yoke running at low-frequency (\ie $\w_{1}=1\,\si{\radian\per\second}$%\mh{\done{Please provide units for $\w_{1}$ and $\w_{2}$. I suppose these are in \si{\radian\per\second}?}}, $\v_{1}= 1-\exp(-(1)^2)$
) and $\NdscotchYokeSimulationHi$ at high-frequency ($\w_{2}=2\,\si{\radian\per\second}$%, $\v_{2}= 1-\exp(-(2)^2)$
). The same procedure is used to collect fabric movement data $\Df$ for lengths $\L\in\{\frac{1}{3},\frac{2}{3},1\}\si{\metre}$ (\ie $\df_{1}$, $\df_{2}$, $\df_{3}$) and rigid body data $\Dr$ (\ie $\dr_{1}$). %\mh{\done{Are these units/parameters correct?}}\mh{\done{How can it be, when there are only $\Nd=2$ data points? (I assume that $\bphi=(\xf(t=0),...,\xf(t=\Tk))^\T$, right?)}}. 
The data is split into equal-sized training and test sets and used to train a \gls{svm} classifier (Libsvm toolbox \cite{chang_libsvm_2011}) to perform \gls{ar} with Gaussian \glspl{rbf} as the kernel function. The \gls{svm} is trained to predict the mapping
\begin{equation}
\bphi_\nd\mapsto\y_\nd
\end{equation}
\edit{in an online fashion, where $\y_\nd\in\{0,1\}$ is the class label ($c=0$ for $\w_1$, $c=1$ for $\w_2$) and $\bphi_\nd$ is the $\nd$th trajectory fragment. }{in an online fashion, where $\bphi_\nd$ is a fragment of the $\nd$th trajectory and $\y_\nd\in\{0,1\}$ is the corresponding class label ($c=0$ for $\w_1$, $c=1$ for $\w_2$).}{mh}
%\mh{\done{What results do you get with a linear basis?}}\ts{\gls{rbf}'s result is better}\mh{\done{Give the parameters used for the \gls{svm}. Describe how they are chosen.}} 
%
Specifically, following \cite{michael2017}, each trajectory is segmented into \edit{windows of size $\Nw$ (where $\Nw < \Nk $ and $\Nk=\Tk/\fk$) , windows overlap by every $i$ time-steps, and predictions are made every single time step}{overlapping windows of size $\Nw$ (where $\Nw < \Nk $ and $\Nk=\Tk/\fk$), }{mh} \ie
\begin{equation}
\begin{split}
\bPhi:&=\left(\bphi_1,\bphi_2,...\bphi_\Nd\right)\\
&=\left((\xf_{1},...,\xf_{\Nw})^\T,(\xf_{2},...,\xf_{\Nw+1})^\T,(\xf_{3},...,\xf_{\Nw+2})^\T,...\right)\edit{}{.}{mh}
\end{split}
	\label{e:bphinsy}
\end{equation}
%\mh{\done{Please fix \eref{bphinsy} as it does not make sense. For instance, if $\Nk=8$, $\Nw=4$, then $\bphi:=[(\xf_{1},...,\xf_{4})^\T,(\xf_{2},...,\xf_{6})^\T,(\xf_{4},...,\xf_{8})^\T,...]$. These have different sizes (\eg $(\xf_{1},...,\xf_{4})^\T=(\xf_1,\xf_2,\xf_3,\xf_4)^\T$ has 4 elements, but $(\xf_2,\xf_3,\xf_4,\xf_5,\xf_6)^\T$ has 5 elements), and you miss points (\eg there is no $(\xf_3,...)^\T$).}}
The procedure is repeated $\TrialsscotchYokeSimulation$ times for each condition and the classification accuracy computed. 
%\mh{\done{I suggest you also compute the precision, recall and F1 scores, and consider presenting as a confusion matrix.}}
\mh{I suggest you release the data and source code used for this evaluation.}%
\mh{Please add the data and source code used for this evaluation to our group github repository.}%
\subsubsection{Results}\label{s:scotch_yoke:results}
\fref{result}\ref{f:result-a} shows the overall accuracy of \gls{ar} using the \gls{svm} classifier with different window sizes. As can be seen, \edit{}{the accuracy is higher when using fabric data at small window sizes. Moreover, the accuracy is higher when $\L$ is greater, in line with the prediction of the model. As the window size increases (\ie the classifier is given more of the trajectory history) the overall accuracy increases and the difference between fabric and rigid data gradually disappears.  }{mh}the accuracy rises \id{do you need to explain this in a little more detail?} 
%\mh{\done{To show this, you would need to plot $\L$ against accuracy.}} 
\edit{with increasing $\L$ in line with the prediction of \eref{DXfXr}. In addition, larger window size means more information are used in \gls{svm} classification, which contribute to achieve higher classification accuracy for each sensor. }{}{mh}
%\mh{\done{You should also comment on the relationship between accuracy and window size.}}
%The \gls{pcc} between \gls{ar} accuracy and the \gls{ks} difference is $0.9718$ revealing a very strong positive correlation.
%\begin{figure}%
%\input{figure/svm_sim}%
%\input{figure/svm_real}%
%\input{figure/vary_frequency}%
%\input{figure/vary_frequency_ks}%
%\caption{Mean accuracy of \ref{f:ma-a} \sref{scotch_yoke} and \ref{f:ma-b} \sref{pendulum} with $100$ trials ($\pm$ standard derivation) when varying window size.}
%\label{f:re}%
%\end{figure}%


%\subsection{Simulation}\label{s:Simulation}\mh{\done{Move the modelling work from \sref{Simulation} to \sref{problem_definition} and use it as a worked example to support your theory.}}
%Given a one dimensional mass-spring-damper system, the position of the mass can be seen as the position of the body under light damping ($\beta<\dot{y}$).\mh{What is $\beta$? Why do you need $\beta<\dot{y}$?} The position of the mass can be computed as the given equation \cite{yang2017basic}:
%\begin{equation}
%w\edit{\ddot{y(t)}}{\ddot{y}(t)}{mh} + \beta %\edit{\dot{y(t)}}{\dot{y}(t)}{mh} + ky(t) = 0
%\label{e:underdamped}
%\end{equation}
%\edit{Where}{where}{mh} $y(t)$ is the position of the mass at time $t$,  $w$ is the weight of the mass, $\beta$ and $k$ are friction coefficient and spring constant respectively.

%Therefore, the \gls{pdf} of each position of the mass [$m_{0}$,$m_{1}$]\mh{In \eref{underdamped} you denote position as $\y$, so do you mean $[\y_{0},\y_{1}]$? If so, what are $\y_{0}$ and $\y_{1}$?} can be seen as\mh{\done{This claim needs back up. Either you need a reference where it has been shown that it is a Gaussian, or you need to present a strong argument as to why it is (or can be approximated to be) a Gaussian.}} Gaussian distribution $P \sim \mathcal{N}(\mu_{1},\sigma_{1})$.\mh{Do you mean $\P(\y)\sim\mathcal{N}(\mu_{1},\sigma_{1})$?} A strip of fabric of length $l$ is attached loosely to the tip of the mass, as would be expected from an item of loose natural clothing.\mh{\done{I suggest you produce a diagram of this.}} As the body moves, the fabric will also \edit{more correlated to}{move alongside}{mh} the mass, but will undergo additional motion due to the complex fabric dynamics. During motion, this attached fabric\mh{\done{If the fabric is of length $l$, this presumably refers to a sensor attached to the \emph{tip} of the strip. Again, a diagram would help here.}} can be in any position within the range [$m_{0}-l$,$m_{1}+l$] with probability $Q \sim \mathcal{N}(\mu_{2},\sigma_{2})$.\mh{\done{The Gaussian has asymptotic tails, meaning that according to this model there is a non-zero (albeit small) probability that the position is outside this range. Therefore you should either (i) make it clear that this is an approximation, or (ii) use a different \gls{pdf} in your model.}} In this, \edit{$\mu_{2}$ and $\mu_{1}$ are the same}{$\mu_{2}=\mu_{1}$}{mh} due the symmetry of Gaussian distribution.\mh{\done{Are they necessarily the same due to the model, or is this an assumption?}} The difference between $\sigma_{2}$ and $\sigma_{1}$ is increasing with the fabric length $l$ is increasing and \edit{$\sigma_{2}$ is no less than $\sigma_{1}$}{$\sigma_{2}\ge\sigma_{1}$}{mh} considering the uncertainty of the fabric movement. The uncertainty of fabric increases with the fabric length \edit{increases.}{}{mh} $\sigma_{2}-\sigma_{1}\propto l\geq0$. Referring the closed-form formula of \gls{kl} between two unfvariate Gaussian distributions \cite{huber2008entropy}, \gls{kl} between the position of the fabric (the loose sensor) and the position of the mass (the body under observation), is given by:\mh{\done{Please provide an explicit derivation of \eref{Simulation} in the appendix.}}
%\begin{equation}
%KL(P||Q) = log{\frac{l+\sigma_{1}}{\sigma_{1}}} + %\frac{\sigma_{1}^2}{2(l+\sigma_{1})^2} - \frac{1}{2}\edit{}{.}{mh}
%\label{e:Simulation}
%\end{equation}
%\mh{Does the $\log$ apply only to the first term in \eref{Simulation}?}
%According to \eqref{e:Simulation}, it is known that \gls{kl} between the position of mass and fabric is rising to infinite when fabric length is increasing (see Fig.~\ref{simulation}(a)),\mh{\done{I suggest you express this in terms of $\lim_{l\rightarrow\infty}KL(P||Q)$.} which predicts that longer fabric length $l$ gradually\mh{From Fig.~\ref{simulation}(a) it looks like $\lim_{l\rightarrow\infty}KL(P||Q)=c$ where $c$ is some constant, which contradicts this argument.}} \edit{improve the hardness}{increases the difficulty}{mh} of \gls{me}.\mh{What about \gls{ar}?}


%To simulate classification between different motions for body-attached sensor and cloth-attached sensor. The mass-spring-damping system uses variety weight $m$ added on the mass expected to generate different motions. The higher added weight $m$ is able to observe the moving pattern of the mass with longer time in one period $T$ as \eqref{mass-spring} shown.
%\begin{equation}
%T = 2\pi\sqrt{\frac{m}{\beta}}
%\label{mass-spring}
%\end{equation}

%Therefore, we also assume $\sigma_{1}$ of its \gls{pdf} is increasing with higher $m$. $\sigma_{1}\propto m$.
%Given the fixed length $l$ of the fabric attached on the mass, the standard derivation of fabric position should be always higher than the mass position. ($\sigma_{2} \textgreater \sigma_{1}$ at any $m$) Then, \gls{kl} between different added mass $m$ for the position of fabric (the loose sensor) and the position of the mass (the body under observation) are given at below. 

%For mass, 
%\begin{equation}
%KL(P||Q) = log{\frac{m+\sigma_{1}}{\sigma_{1}}} + %\frac{\sigma_{1}^2}{2(m+\sigma_{1})^2} - \frac{1}{2}
%\label{e:Simulation1}
%\end{equation}

%For fabric, 
%\begin{equation}
%KL(P||Q) = log{\frac{m+\sigma_{2}}{\sigma_{2}}} + %\frac{\sigma_{2}^2}{2(m+\sigma_{2})^2} - \frac{1}{2}
%\label{e:Simulation2}
%\end{equation}
%\mh{Please provide an explicit derivation of \eref{Simulation1} and \eref{Simulation2} in the Appendix.}
%\ts{I am trying to use JS to represent classification and regression in simulation, but theory is here.}

%Comparing between \eqref{e:Simulation1} and \eqref{e:Simulation2}, it is seen that \gls{kl} on the position of fabric invariably higher than the position of the mass. (see Fig.~\ref{simulation}(b)) This indicates that for any speciﬁc mass, the fabric sensor shows a greater independence than the body sensor, and as such, would be more suited to \gls{ar}. 

\stepcounter{casestudy}%
\subsection{Case Study \thecasestudy: Scotch yoke}\label{s:scotch_yoke}
%\subsection{Experiment Setup}
\label{s:Experiment}
%\subsubsection{Data Acquisition}
\label{s:data_acquisition}
This evaluation aims to validate the proposed framework \edit{when performing \gls{ar}}{}{mh} in a \emph{physical system}. \edit{The procedure is as follows.}{}{mh}
\subsubsection{Materials and Methods}\label{s:scotch_yoke:mnm}
To ensure accurate and repeatable data collection, the experiment reported here uses an instrumented \emph{scotch yoke} as a data acquisition device. %, as an approximation of the shank of an adult human leg with a loose, sensorised garment attached.
%
%\ts{\done{Do we really need three parameters? I think we just need sensor position as we know sensor F3 can generate obvious more amount of noise than F2, R1 has no noise. So, it is simple to know longer length, more motion artifacts. The stiffness of three fabric materials in this experiment has no obvious different and may not be able to change the conclusion and they also have different structures to make this theory more complicated. So, I could keep rigid pendulum data and one of fabric data.}}
%\mh{My concern is that a reviewer might raise the criticism that your analysis is only for one fabric type (so may not generalise to others). However, I agree, it makes the story more complex, so for the time being, I am happy for you to centre your analysis on just one fabric type. We can decide whether to include further fabric types later on.}
%
The experimental setup is shown in \fref{setup}\ref{f:setup-c}. The actuated scotch yoke consists of a sliding yoke, with rigid rods affixed either side and a rotating disk of diameter $\SI{20}{\cm}$ mounted on two bearing blocks and driven by a DC motor with encoder ($30:1, 37D$ gear-motor, Pololu Corporation, USA) at the fulcrum. The motion of the disk and yoke are coupled via a sliding pin, ensuring a pure sinusoidal movement of the \edit{latter}{yoke}{mh}. Affixed to the \edit{sliding yoke}{latter}{mh}, $\SI{10}{\cm}$ away from the fulcrum, is a \SI{30}{\cm}$\times$\SI{5}{\cm} %\mh{\done{Check your measurements: according to \fref{sp} the fabric is \SI{36}{\cm} long.}} 
strip of woven cotton fabric %\mh{\done{The fabric you are using is not jersey (if it is, it should be knitted, and stretchy, see \texttt{https://en.wikipedia.org/wiki/Jersey\_(fabric)}). It seems to be woven cotton.}}
upon which are mounted three sensors (NDI Aurora Magnetic Tracking device, NDI, Canada) that synchronously record the horizontal position \edit{with position errors is approximately $0.09\si{\mm}$}{}{mh} %\mh{\done{It is better just to state the measurement accuracy. Please add this here.}}
at $\SI{40}{\Hz}$\edit{}{, at an accuracy of approximately $0.09\si{\mm}$}{mh}. The latter are attached along the length of the fabric\edit{,}{}{mh} \il{\item $\SI{20}{\cm}$ \edit{from the fulcrum}{}{mh} ($\df_{2}$)\edit{}{,}{mh} \item $\SI{30}{\cm}$ \edit{from the fulcrum}{}{mh} ($\df_{3}$) and \item \edit{at the tip of the fabric}{}{mh} $\SI{40}{\cm}$ from the fulcrum ($\df_{4}$) \edit{}{(\ie at the tip of the fabric)}{mh}.} \id{\done{non sure what is the difference between (i) and (ii)}} A further sensor \edit{}{($\dr_{1}$) }{mh}is rigidly attached to the yoke at the fabric attachment point \edit{$\dr_{1}$}{}{mh} (see \fref{setup}\ref{f:setup-c}). \edit{Note that, due to its construction, there are some unavoidable factors that affect the quality of the collected data (\eg air resistance, friction between components, slight non-alignment of the yoke movement with the reference frame of the motion tracker). Using the rigidly attached sensor ($\dr_{1}$) as a reference against the theoretical predictions of \eref{xr} the error of movement frequency is approximately}{The error in the yoke movement against the sinusiodal reference is}{mh}\footnote{The detail is provided in \sref{rmse}.}\mh{Avoid placing footnotes where they might clash with superscripts in mathematics. I have moved this one for you.} $\pm 0.05\pi\si{\radian\per\second}$.
\mh{It would be better to cite the RMSE not the \gls{mse} - since the units of RMSE will be \si{\mm}. Please provide a full account of how you estimated this error, and the exact errors you computed, in the appendix.}\id{do you need to say how this was calculated? i.e. give more detail, as this was something that we discussed in our last meeting}
%\begin{figure}
%\input{figure/setup}%
%\caption{Front-view of the experiment set up. Sensors are placed \il{\item at equidistant intervals along the fabric strip ($\df_{2}$-$\df_{4}$) and \item rigidly at the attachment point ($\dr_{1}$)}.}
%\label{f:sp}%
%\end{figure}%
%\mh{\done{\fref{sp}: The mechanism is very hard to see as it is all black on a black background. Please take a better picture.}}
%\mh{\done{\fref{sp}: The background of this image is cluttered and it can be hard to see what is part of the set up. I suggest you retake the photo with a plain background (we have drapes you can use for this).}}
%\mh{\done{\fref{sp}: I suggest you combine \fref{mb} with this figure to have 3 panels side-by-side.}}
%\edit{Two modes have been applied. \il{\item Passive pendulum mode: pendulum is raising to the horizontal position on the left hand side and releasing it to swing in gravity. $\SI{40}{\gram}$ weights are added to the tip of the pendulum to increase swing speed. \item {Actuated pendulum mode: this is to simulate the various patterns of shank movement. DC motor with encoder ($37D$ gear-motor, Pololu Corporation, USA) is installed at the tip of the pendulum used to control the swing speed and direction of the pendulum}}. In the experiment reported below, the tip of the fabric ($\SI{20}{\cm}\times\SI{5}{\cm}$ strip of jersey) is affixed to the pendulum at $\SI{10}{\cm}$ away the pivot. $3$ sensors are attached on the rigid pendulum and anther $3$ sensors are attached on the piece of fabric with corresponding position. These sensors are denoted as \il{\item $F1/R1$ ($\SI{15}{\cm}$ from the pivot), \item $F2/R2$ ($\SI{20}{\cm}$) and \item $F3/R3$ ($\SI{25}{\cm}$)} (See Fig.\ref{f:diagram}).}{}{mh}
%\begin{figure}[htbp]
%\centerline{\includegraphics[height=0.5\linewidth]{diagram.eps}}%
%\caption{Schematic of experimental setup.}
%\label{f:diagram}
%\end{figure}
%\mh{\done{I suggest you add an annotated photograph of your experimental setup to \fref{diagram}.}}
%\mh{Please improve the quality of \fref{diagram} to a standard consistent with \fref{pro}.}
%
%\mh{Give the parameters of the pendulum, \ie mass, length, \etc. Are these a reasonable approximation of the human lower-leg?}\mh{Give the dimensions of the fabric. If you are not using roma in the analysis, please replace with the appropriate one.}
%\edit{The data is collected with NDI Aurora Magnetic Tracking device (NDI company, Canada) that synchronously samples data from Aurora sensors (NDI company, Canada) recorded at $\SI{40}{\Hz}$. Each data point contain position information of the sensor at two dimensions (horizontal and vertical).}{}{mh}
%\id{did you really compare your accelerations with and without weight with those experienced in walking and running}
%\id{you need to be very specific when you propose the pendulum as a proxy for shank motion. I understand that you say that the pivot corresponds to the knee joint, but this is an approximation. is the length comparable? does it matter that you have 18cm of fabric distal to the pendulum. you need to better describe and justify your model. Every model has its limitations and it is not perfect, so this is not a problem, but you need to show that you have considered the limitations and you can interpret your results accordingly }

With this set up, data is collected from the device driven at \emph{low} ($\w_{1} = 1.05\pi\,\si{\radian\per\second}$) and \emph{high} ($\w_{2} = 1.48\pi\,\si{\radian\per\second}$) speeds.\footnote{\label{fn:missing-data} Note that, at high speeds NDI device occasionally loses track of its sensors resulting in missing data (\ie gaps) within trajectories. These are filled using piecewise cubic spline interpolation.}. \Numberstringnum{\NdscotchYokeExperiment} sample trajectories of length $\Tk=$\SI{5}{\second} at each speed are recorded. %\mh{\done{Specify trajectory lengths.}}%\mh{\done{Please check units for $\w_{1}$ and $\w_{2}$. I suppose these should be in \si{\radian\per\second}.}}
%Wherever this occurs in this experiment, the trajectory is discarded and replaced with the next complete trajectory collected.}} for $\Tk=\SI{\TkscotchYokeExperiment}{\second}$. This is repeated until\FPeval{\ans}{clip(\NdscotchYokeExperiment)} \ans\ sample trajectories for each category are recorded.
%
%{This procedure is repeated with a $\SI{40}{\gram}$ weight affixed to the distal tip of the link to produce an equal number of \emph{fast-swing} trajectories ($\y=1$), resulting in a total of $\Nd=\NdPendulumExperiment$ sample trajectories.}{mh}              
%
%\mh{At this point, the data for one trial consists of $\D=\{\{\brddotRi,\brddotFii,\brddotFiii\}_{\nd=1}^\Nd,\c\}$ where $\Nd=\SI{5}{\second}\times\SI{600}{\Hz}=3000$ data points, $\brddot_i=(\rddoti,\rddotii,\rddotiii)_i^\T$ is the tri-axial acceleration for sensor $i$ and $\c\in\{0,1\}$ is the class label for the movement (\ie non-weighted or weighted, respectively).} 
%
%\mh{\done{I would expect a description of how this data is used to compute \gls{mi} to appear here. What (if any) assumptions are used? How do you go from the raw data, to the quantities described in \eref{mi}-\eref{MI}?}}
%
%
%\subsubsection{Signal unit conversion}
%It is necessary to use standard acceleration unit (\eg $m/s^{2}$) instead of raw data in signal analysis. Therefore, this shows the procedure to convert from matrix $\sigma$. First of all, Place sensor so that $X-axis$ is orthogonal to earth's gravity, and note the value $(480)$ and place sensor upside down (still so that $X-axis$ is orthogonal to earth's gravity)and note the $(300)$ value. Therefore, it is found that $[-1g,1g]$ in gravity acceleration unit is corresponding with its raw data $[300,480]$. Then, to covert it, it needs to map the raw date to gravity unit acceleration range as equation \eqref{map} shows below.
%\begin{equation}
%f(\sigma) \mapsto f(\psi), \sigma\in[300,480], \psi\in[-1g,1g]
%\label{map}
%\end{equation}
%Where $\sigma$ and $\psi$ define the range of raw data and acceleration sensor measurement scale respectively. $g$ represents gravity, $g=9.8$ is used in calculation.
%
%\subsubsection{Signal time alignment}
%All samples of acceleration signal are time-aligned, based on setting the threshold as the amplitude of the signal decreases significantly released from static condition. Two thresholds $(460, 360)$ are chosen for tangent acceleration $(\rddot_{z})$ and centripetal acceleration $(\rddot_{y})$ respectively, which can be described by equation \eqref{time}.
%
%\begin{equation}
%\begin{split}
%\mathbf{\rddot}= \left \{
%\begin{array}{ll}
%   0              & \mathbf{\rddot}_{z}>460\\
%\mathbf{\rddot}_{z}      & \mathbf{\rddot}_{z}\le460\\
%   0              & \mathbf{\rddot}_{y}>360\\
%\mathbf{\rddot}_{y}  & \mathbf{\rddot}_{y}\le360\\
%\end{array}
%\right.
%\end{split}
%\label{time}
%\end{equation}
%
%\subsubsection{signal Scaling}
%After the conversion, the converted acceleration signal $(\psi)$ also need to be scaled with the purpose of making indicators of different units or magnitudes can be compared and avoiding complicated numerical calculation \cite{hsu2003practical}. This procedure is mapping the acceleration signal with the gravity unit $m/s^{2}$ to the normalized range $[-1,1]$ as described in equation \eqref{mapto}.
%
%f(\psi) \mapsto f(\upsilon), \upsilon\in[-1,1]
%\label{mapto}
%\end{equation}
%Where $\upsilon$ means normalized range.
%
%\subsubsection{Fill missing data}
%The NDI device may not capture data when pendulum is swinging with high acceleration, the missing data is replaced using a moving median with a window of length $15$.
%\subsection{Signal Processing}
%
%\subsubsection{Remove the missing data}
%\edit{The NDI device used in this experiment may loss data when the pendulum experiences fast-swing acceleration. Therefore, simply remove the missing data.}{}{mh}\mh{I have moved this to footnote \ref{fn:missing-data}. Please confirm that this accurately describes how you handled missing data.}
%\subsubsection{Signal segmentation}
%\edit{It is known that fabric-attached sensors are not contain the same amount of additional information during the full swing period. To ensure the processed data contain certain amount of additional information, the data $\sigma$ is segmented into several intervals with number of $n$ points as window size. These windows can be defined as subsets of full trajectory signal shown as follow. In this study, $n$ is set as $20$.}{}{mh}
%\begin{equation}
%\edit{\sigma: = [(\phi_{1},...\phi_{n})^\mathrm{T}, (\phi_{n+1},...\phi_{2n})^\mathrm{T},...,(\phi_{200-n},...\phi_{200})^\mathrm{T}]}{}{mh}
%\label{Segment}
%\end{equation}
%\ts{I have no idea whether I should segment data or use whole trajectory to do classification}\mh{I suggest you first try using the whole trajectory as the input feature, \ie  $\bphi_\nd=(\xf(t=0),...,\xf(t=\Tk))^\T$ where $\bphi_\nd$ is the $\nd$th column of $\bPhi$, the feature matrix. It doesn't make much sense to me to segment in the way that you describe in (\ref{Segment}), since later segments will have little similarity to earlier ones.}
%
%\subsection{Signal Analysis}
%\edit{The collected signal matrix $\sigma$ are analysed to compare between the performance of rigid-attached sensors and fabric-attached sensors. Comparisons are also made across different motions (\eg slow-swing and fast-swing) through two types of behaviour analysis tasks. The signals are analysed in MATLAB R2020b (MathWorks, USA). }{}{mh}
%
%\subsubsection{\Acrlong{ar}}\label{s:activity_recognition}
%\edit{Specifically, the \emph{\acrlong{ar}} task involves using the sensor signals to predict the class label (\ie \emph{slow-swing} ($\alpha$) or \emph{fast-swing} ($\beta$)), \ie the mapping}{}{mh}
%\begin{equation}
%\edit{\{\phi_{i}\}_{\nd=1}^\alpha\mapsto\{\c_i\}_{\nd=1}^\alpha = 0}{}{mh}
%\end{equation}
%\begin{equation}
%\edit{\{\phi_{i}\}_{\nd=1}^\beta\mapsto\{\c_i\}_{\nd=1}^\beta = 1}{}{mh}
%\end{equation}
%\edit{where $\phi_{i}$ is data sample collected from sensor $i$ ($i\in\{R_{1},R_{2},R_{3},F_{1},F_{2},F_{3}\})$.}{}{mh}
%
%\subsubsection{\Acrlong{me}}\label{s:motion_estimation}
%\edit{The \emph{\acrlong{me}} task involves using the sensor signals to predict salient features of the movement. Here, interest focuses on predicting body movement from the fabric-mounted sensors \ie the mapping}{}{mh}
%\begin{equation}
%\edit{\{\phi_{F_{i}}\}_{\nd=1}^\Nk\mapsto\{\phi_{R_{i}}\}_{\nd=1}^\Nk}{}{mh}
%\end{equation}
%\edit{where $\phi_{i}$ is collected from sensor $i\in\{1,2,3\}$.}{}{mh}
%
%\subsubsection{Support vector machine}
%This data is used to train a \gls{svm} classifier with the \gls{rbf} kernel. In terms of cross-validation, it uses five-fold cross-validation. For grid search, it is used to find optimal value for two parameters ($C$ and $\gamma$). Range $2^{-5}$ to $2^{5}$ is chosen for $C$ and $\gamma$ in classification after coarse grid. %\mh{\done{Is this also done when computing the \gls{mi}? If so, it is a general post-processing step, so belongs in \sref{data_acquisition}.} }
%
This data is segmented for online learning through a similar procedure as described in \sref{scotch_yoke}, randomly split into equal-sized training and test sets\edit{}{,}{mh} and used to train a \gls{svm} classifier to perform \gls{ar}. All data are \edit{standardized}{standardised}{mh} using \edit{}{the }{mh}$z$-score. %computed by: 
%\begin{equation}
%    \xf_{z}=\frac{\xf-\mu}{\sigma}
%\end{equation}
%\mh{\done{I do not understand this (preceding) sentence.}} 
The performance of the classifier is assessed by computing \edit{the}{its}{mh} accuracy and the \gls{ks} test statistic via \eref{ks_def}. This process is repeated for $\TrialsscotchYokeExperiment$ trials of every experimental condition tested.
%\providecommand{\bphiX}{{\color{mh}Define \textbackslash bphiX}}

%In \gls{me}, each point consists of the tuple $[\bPhi_\nk,\by_\nk]$, where $\bphi_{\alpha}, \bphi_{\beta}\in\bPhi_\nk$ is the $\nk$th sample of the instantaneous position information from the fabric sensor of interest (\ie $F_{1}$, $F_{2}$ and $F_{3}$) and $\bphi_{\alpha}, \bphi_{\beta}\in\by_\nk$ is the $\nk$th sample of the instantaneous position information from the rigid sensor (\ie $R_{1}$, $R_{2}$ and $R_{3}$) considered as target. The complete data set provided to the regressor would then be $\bPhi=[\phi_{1}^{\alpha},...,\phi_{\dimphi}^{\alpha},\phi_{1}^{\beta},...,\phi_{\dimphi}^{\beta}]\in\mathbf{R}^{400\times2}$, $\by=[\by_{1}^{\alpha},...,\by_{\dimphi}^{\alpha},\by_{1}^{\beta},...,\by_{\dimphi}^{\beta}]\in\mathbf{R}^{400\times1}$ for each dimension in the target $\by$. To the end, it uses the following equation to include both dimensions.
%\begin{equation}
%r^{2} =\frac{r^2_{x} +r^2_{y}}{2}
%\label{r2}
%\end{equation}
\subsubsection{Results}\label{s:scotch_yoke_experiment_results}
\fref{result}\ref{f:ma-b} shows the accuracy of \gls{ar} using the \gls{svm} classifier for window sizes $0.025\le\Nw\edit{}{/\fk}{mh}\le2.5\,\si{\second}$. \edit{As can be seen, for all window sizes, the accuracy is higher using data from fabric-attached sensors than rigid attached sensor. Specifically, the classification accuracy from high to low is  $\df_{4}$, $\df_{3}$, $\df_{2}$, $\dr_{1}$, which is consistent with the prediction of \eref{DXfXr}.}{A similar, but more pronounced trend is seen here as for the simulation: the accuracy is higher for fabric-attached sensors at small window sizes (and higher for sensors at greater $\L$). As the window size increases, the accuracy converges toward the same value, regardless of the sensor used.}{mh}
%
%\subsubsection{Similarity measurement}
%The estimation of \gls{js} is based on test dataset in \gls{svm}. We let data $\varphi_{1}^{10} = [\phi_{n+1}^,...,\phi_{2n}]\in\mathbf{R}^{200\times2}$. The following is describing how to estimate \gls{js}. The first step is applying \gls{em} algorithm. This algorithm is used to fit the parameters of the \gls{gmm} since data can be seen as a \gls{gmm}. This is iterations algorithm. In each iteration, it consists of the \emph{Expectation} step (E-step) and the \emph{Maximization} step (M-step). Details of two steps are describing below. 
%
%\gls{js} is used to measure similarity. Generally, \gls{js} is symmetric $\gls{js}(\Xf_{\w=1}:\Xf_{\w=2}) = \gls{js}(\Xf_{\w=2}:\Xf_{\w=1})$, and its value is strictly bounded between $0$ and $1$ if using the base $2$ logarithm in the computation $0 \leq \gls{js}(\Xf_{\w=1}:\Xf_{\w=2})\leq 1$. \gls{js} is $0$ if two probability distributions are completely the same. While \gls{js} is $1$ if two probability distributions are completely different.
%\gls{js} can be expressed as \cite{nielsen2020generalization}.
%\begin{equation}
%\begin{split}
%& \gls{js}(\Xf_{\w=1}:\Xf_{\w=2}) =\\ &H\left(\frac{P(\Xf_{\w=1})+P(\Xf_{\w=2})}{2}\right) - \frac{H(P(\Xf_{\w=1}))+H(P(\Xf_{\w=2}))}{2}
%\label{e:js} 
%\end{split}
%\end{equation}
%
%Equation \eref{js} is used to compute \gls{js} between two different of frequency for each sensor measurement.
%
%\gls{ks} test is employed to measure statistical distance. The maximum difference $\Dd$ of test sets of \gls{svm} is computed using equation \eref{ks_def}. 
\tref{ks} shows \edit{the \gls{ks} test $\Dd$-value}{$\Dd$ from the \gls{ks} test}{mh} for each sensor. \edit{it reveals motion artifact from fabric movement can significantly increase statistical distance (\ie $\Dd$). Moreover, more motion artifact, greater statistical distance. These results reveal that there is positive relationship between $\Dd$-value and classification accuracy.}{As can be seen, the statistical distance $\Dd$ is larger for the fabric sensors, and increases with $\L$.}{mh}  
\mh{There is not enough information here to understand what exactly is being reported in this section or what it adds to the analysis. For instance, what is the window size? How is the \gls{cdf} estimated? Why is the increase in $\Dd$ not reflected in the accuracy? I suggest you drop this and remove \fref{ks} unless there is a strong justification to include it.}
\ts{I use the whole signal to compute ks test D. The signal is not sliced. So there is no window size. I used Matlab function 'kstest2' to compute. It used histogram to compute cdf.  }
\mh{It is still unclear what this adds to the analysis. What can we see in \tref{ks} that we can't in \fref{result}?}
\begin{table}%
\input{figure/ks}%
\caption{\edit{Mean \gls{ks} test statistic $\Dd$ with $100$ trials ($\pm$ standard derivation) for each sensor.}{\Gls{ks} test statistic $\Dd$ computed on data from each sensor in the physical scotch yoke (mean$\pm$s.d. over trials).}{mh}}
\label{t:ks}%
\end{table}%
\mh{\fref{ks}: Unclear what this is showing - suggest removal.}
%\mh{\done{\fref{ks}: Bar chart is only showing 4 numbers (8 if you include the s.d. values) - these could be more compactly included as a table, or in line with the text.}}
\mh{\tref{ks}: Ensure each number has the same number of decimals.}
\mh{\tref{ks}: Unclear which window size this refers to (presumably, the smallest?)}
\mh{Reviewed to here 31/8/2022.}%
\subsection{Classification with varying frequency}
To investigate the effect the difference in two motion speeds (\ie $|\w_{2}-\w_{1}|$) has on this result, the experiment is repeated varying the high-speed motion $1.26\pi\le\w_{2}\le1.48\pi\,\si{\radian\per\second}$.
\mh{\done{It is odd that there are irregular intervals between the $\w_{2}$ in this experiment. Can you justify this?}}
\mh{\done{Why is it that only $\df_{4}$ seems to show improvement over $\dr_{1}$ in this experiment?}}
\mh{It would be interesting to see how $\Dd$ changes for each pair of $\w_{1}$ and $\w_{2}$ tested, and whether this reflects the model predictions.}
\subsubsection{Results}
\begin{figure}%
\input{figure/svm_sim}%
\input{figure/svm_real}%
\input{figure/vary_frequency}%
\input{figure/vary_frequency_ks}%
\caption{\edit{Mean accuracy of }{Recognising movements of different frequency in  the }{mh}\cl{\item\label{f:result-a} \edit{\sref{sim}}{simulated}{mh} and \item\label{f:result-b} \edit{\sref{scotch_yoke}}{physical scotch yoke}{mh} \edit{with $100$ trials ($\pm$ standard derivation)}{(mean$\pm$ s.d. over $\TrialsscotchYokeSimulation$ trials)}{mh} when varying window size. Mean \item \label{f:result-c} classification accuracy and \item \label{f:result-d} \gls{ks} test statistic $\Dd$ between $0.95\pi/s$ with each frequency $100$ trials ($\pm$ standard derivation) when window size is $0.025s$.}}
\label{f:result}%
\end{figure}

\ts{I have updated equation 6(z1,z2). The result should be correct. I have tried with cross-validation and grid search.}
%\begin{figure}%
%\input{figure/vary_frequency_ks}%
%\caption{Mean \gls{ks} test statistic $\Dd$ between $0.95\pi/s$ with each frequency $100$ trials ($\pm$ standard derivation).}
%\label{f:vary2}%
%\end{figure}%
\mh{\done{\fref{vary}: I do not advise including this figure, unless you are able to explain the apparent anomaly at $\w_{2}=1.4\pi\,\si{\radian\per\second}$. You risk being accused of cherry-picking your results in \sref{scotch_yoke_experiment_results} by choosing the case that shows the biggest difference.}} \id{\done{not sure that I understand figure 9 and its explanantion. I suggest adding legends, and you did not say anything about the peak at 1.4, unless I missed it, I do not see a clear explanation of the data, you seem to imply a 'linear increase', but this is not the case, I think}}
\fref{result}\ref{f:result-c} and \fref{result}\ref{f:result-d} show the classification accuracy and \gls{ks} test statistic D for discriminating between $\w_{1}=1.05\pi\,\si{\radian\per\second}$ and the different $\w_{2}$ when $\Nw=\SI{0.025}{\second}$ respectively.
\mh{\done{It would be better to choose the window size as one of those shown in \fref{real} so that the reader can compare the results.}} 
As can be seen, the larger difference between two movement frequencies, data collected from fabric-attached sensors have higher performance of \gls{ar} and greater statistical distance. For rigid-attached sensors, there is no obvious increase for classification accuracy and statistical distance (\ie $\Dd$) when using larger difference in two motions. Those are consistent with the prediction of \eref{DXfXr}. 
\mh{\done{More explanation of the results needed, especially why the result at $\w_{2}=1.4\pi\,\si{\radian\per\second}$ is out of line with the trend.}}
\mh{\done{It seems that the results for $\df_{2}$ and $\df_{3}$ are no better than for $\df_{4}$. How do you explain this?}}

%From this test dataset, the joint probability distribution is $P(\eta_{i},z_{i};\theta_{i})$, the conditional probability distribution is $P(\eta_{i},z_{i}|\theta_{i})$ and maximum iteration $J_{max} = 1000$. In this, $\theta$ is Gaussian parameters $N(\mu,\Sigma)$ and $z$ is the latent variable.  initial parameters $\theta$ and iteration begins $J = 1, 2,...,J_{max}$.  

%E-step: Compute likelihood estimation $l(\theta,\theta_j)$ as equation \eqref{e2}. 

%\begin{equation}
%Q_i(z_i) = \P(z_i|\eta_i,\theta_i)
%\label{e1}
%\end{equation}

%\begin{equation}
%l(\theta,\theta_j) = \sum_{i=1}^{n}\sum_{z_i}\P(z_i|\bphi_i,\theta_i)log(\frac{\P(\bphi_i,z_i;\theta)}{\P(z_i|\bphi_i,\theta_i)})
%\label{e2}
%\end{equation}

%where $P(\bphi_{i},z_{i};\theta_{i})$ is the joint probability distribution, $P(\bphi_{i},z_{i}|\theta_{i})$ is the conditional probability distribution, $\theta$ is Gaussian parameters $N(\mu,\Sigma)$ and $z$ is the latent variable.

%M-step: Maximize likelihood estimation $l(\theta,\theta_j)$ shown as as equation \eqref{m}. 
%\begin{equation}
%\theta_{j+1} = \mathop{\arg\max}\limits_{\theta} l(\theta,\theta_j)
%\label{m}
%\end{equation}

%The maximum iteration is $J_{max} = 1000$. Stop iteration if $\theta_{j+1}$ is convergence. Otherwise repeat from E-step. We aims to split into $10$ single Gaussian components. To the end, the output is $\omega_{i=1}^{10}$ and $\theta_{i=1}^{10}(\mu_i,\Sigma_i)$ from one \gls{gmm}. In this, $\mu$ and $\Sigma$ are $2\times 1$ vector and $2\times 2$ matrix respectively. 

%Then, the \gls{pdf} of \gls{gmm} $\P(\varphi)$ can be obtained by the following equation.

%\begin{equation}
%\P(\varphi|\theta_{i}) = \frac{1}{\sqrt{2\pi\Sigma_{i}}}\exp(-\frac{1}{2}(\bphi-\mu_{i})^\mathrm{T}\Sigma_{i}^{-1}(\bphi-\mu_{i}).
%(x-\mu)\Sigma^{-1}(x-\mu)^\mathrm{T})\edit{}{.}{mh}
%\label{e:pdf} 
%\end{equation}

%\begin{equation}\label{e:gmm}
%\P(\varphi) = \sum_{i=1}^{10} \omega_{i} \P(\varphi|\theta_{i})
%\end{equation}\mh{\done{Upper limit of the sum in \eref{gmm} should not be $i$.}}

%Then, entropy of event $\bphi$ can be computed as \eqref{e:entropy} \cite{shannon1948mathematical}.
%\begin{equation}
%H(\varphi)=-\sum \P(\bphi_{i})log_{2}\P(\bphi_{i}).
%\label{e:entropy}
%\end{equation}


%\mh{\done{\eref{entropy} is the entropy for a \emph{continuous-valued} random variable, whereas the text describes a \emph{discrete} set of outcomes. Which is correct?}}
%\mh{\done{The integration limits in \eref{entropy} don't make sense.}}
%Finally, \gls{js} can be computed as following equations \cite{nielsen2020generalization}.

%\begin{equation}
%JS(P||Q) = H(\frac{ \P(P) + \P(Q)}{2}) - \frac{H(P)+H(Q)}{2}
%\label{js} 
%\end{equation}


%where $P$ and $Q$ represent slow-swing motion $\bphi_{1}^{\alpha}$ and fast-swing motion $\bphi_{1}^{\beta}$ in \gls{ar}. For \gls{me}, $P$ and $Q$ donate fabric-attached sensors measurement $(\{\phi_{F_{i}}\}_{\nd=1}^\Nk)$ and rigid-attached sensors measurement $(\{\phi_{R_{i}}\}_{\nd=1}^\Nk)$.


%Generally, the value of \gls{js} is symmetric $JS(P||Q) = JS(Q||P)$, and its value is strictly bounded between $0$ and $1$ if using the base $2$ logarithm in the computation $0 \leq JS(P||Q)\leq 1$ \cite{nielsen2020generalization}, which is the same as the range of classification accuracy ($[0\%,100\%]$) in \gls{ar} and r-squared ($[0,1]$) in \gls{me}. 


%This property \highlight{matches}{mh} with classification accuracy ($[0\%,100\%]$) in \gls{ar} and R-squared\mh{Notation conflict: $R$ is previously used to denote the rigidly-attached sensor.} ($[0,1]$) in \gls{me}.


%\mh{\done{What is the precise meaning of \emph{matches} here? Can you formally show a relationship? Or is it just analogous?}}

%The value of \gls{js} is zero only if \P(P) and \P(Q) are completely the same. While it gets one when they are thoroughly different. This can predict that higher \gls{js} refers to achieve greater classification accuracy in \gls{ar} or poor estimation performance in \gls{me}.


%In the task of \gls{ar}, $P(x)$ and $Q(x)$ \edit{donate}{denote}{mh} two data distributions collected from similar activities (\eg walking and running). Higher \gls{js} refers to different data distributions between two classes, which expect to achieve higher classification accuracy. 

%In the task of \gls{me}, it uses $Q$ as approximate distribution model (\eg cloth movement) to estimate the target $P$ (\eg actual human movement). Higher \gls{js} represents different data distributions between target and data means poor estimation performance (lower R-squared ($R^{2}$)).\mh{A diagram or worked example for the (i) \gls{ar} and (ii) \gls{me} case would help make this clearer and more convincing.}

%Then, taking $\theta_{i}$ into equation \eqref{gmm} and \eqref{pdf} to compute probability density function of mixture of Gaussian. Finally, combing equation \eqref{entropy} \eqref{js} to estimate \gls{js}.


%\subsubsection{Estimating \gls{mi}}
%This is the description how \gls{mi} is computed. Given two vectors $X$ and $Y$. In the calculation of entropy, $P(X)$ is marginal probabilities of $X$, which can be calculated according to histogram. In detail, the intervals is determined according to equation \eqref{intervals}. 
%\begin{equation}
%T_{X} = \frac{max(X)-min(X)}{n},
%T_{Y} = \frac{max(Y)-min(Y)}{n}
%\label{intervals}
%\end{equation}
%Where $T_{X}$ and $T_{Y}$ means the intervals of $X$ and $Y$ respectively, and $n$ is the size of vector $X$ or $Y$.

%Then, the $x-axis$ of the histogram can be obtained. 
%The occurrence of each element in $X$ at each interval can be calculated after plotting its histogram. The marginal probabilities at each interval for vector $X$ and $Y$ can be calculated by equation \eqref{mass}.
%\begin{equation}
%P(X)_{i=1}^{n} = \frac{w_{i=1}^{n}}{n}
%\label{mass}
%\end{equation}
%Where $w$ is the number of occurrence at each interval and $P(X)_{i=1}^{n}$ represents marginal probabilities at each interval.

%Then, entropy can be computed by equation \eqref{entropy}. The joint probability $P(X,Y)$ can be seen as the number of two vectors $X,Y$ falling into the $n*n$ equally divided grid at the same time. Then, the marginal probabilities for $n*n$ of $X$ and $Y$ can be obtained after plotting the histogram and calculated by equation \eqref{joint_mass}.
%\begin{equation}
%P(X,Y)_{i=1*1}^{n*n} = \frac{q_{i=1*1}^{n*n}}{n}
%\label{joint_mass}
%\end{equation}
%Where $q$ is the number of occurrence at each interval within table $n*n$ and $P(X,Y)_{i=1*1}^{n*n}$ represents marginal probabilities at each interval within $n*n$.
%Then, joint entropy can be calculated by equation \eqref{joint_entropy}. Finally, $H(X)$, $H(Y)$ and $H(X,Y)$ are known, $H(X|Y)$ can be simply calculated using equation \eqref{mi}.

%Using completely the same test dataset in method of \gls{svm} to calculate their \gls{mi} for \gls{ar} and \gls{me}. This is to make sure two methods evaluate totally the same data to make the comparison between two methods meaningful.

%\mh{It does not make sense that there are as many class labels ($\Upsilon$) as data points ($\Pi$). Your data contains $\Nk=20$ movements, where each movement is associated with a class label (\ie movement $\nk=1$ has class label $\c=\c_1$ - if this movement is one where the pendulum is non-weighted, then $\c_1=0$, otherwise $\c_1=1$).}
%\mh{I cannot understand why $\Pi\in\mathbf{R}^{2402\times6\times4}$. For the \gls{ar} task, you have $\Nk=20$ sample movements. Each sample contains $\SI{5}{\second}$ of data, \ie $\Nd=3000$ points. If you are doing batch-wise classification, this would translate to $\Nk=20$ data points, where each point consists of the tuple $(\bphi_\nk,\c_\nk)$, where $\bphi_\nk\in\R^\dimphi$ is the feature vector consisting of the instantaneous acceleration in each dimension at each time step, \ie $\dimphi=3\times3000=9000$. The complete data set provided to the classifier would then be $\bPhi=[\bphi_1,...,\bphi_\Nk]\in\R^{9000\times20}$ and $\bc=(\c_1,...,\c_\Nk)\in\R^{20}$ (assuming no validation/test data is held out). Are you sure you have your classification approach set up correctly?}


%\mh{I cannot understand why $\Pi\in\mathbf{R}^{1201\times6\times4}$. For the \gls{me} task, you have a total of $\Nm=\Nk\times\Nd=20\times3000=60000$ data points for each sensor. If you are doing a simple point-wise regression, \ie fitting a model $\by=f(\bphi)$, this would translate to $\Nm=60000$ data points, where each point consists of the tuple $(\bphi_\nm,\by_\nm)$, where $\bphi_\nm\in\R^3$ is the $\nm$th sample of the instantaneous acceleration from the fabric sensor of interest (\ie $\brddotFii$ or $\brddotFiii$) and $\by_\nm\in\R^3$  is the $\nm$th sample of the instantaneous acceleration from the rigid sensor (\ie $\brddotRi$). The complete data set provided to the regressor would then be $\bPhi=[\bphi_1,...,\bphi_\Nm]\in\R^{3\times60000}$ and $\bY=(\by_1,...,\by_\Nm)\in\R^{3\times60000}$. Are you sure you have your regression approach set up correctly?}


%\mh{There is no information on how \gls{mi} is computed in the experiments. What do the random variables $X$ and $Y$ correspond to in your experiment? What do you do to deal with the fact that you don't have access to $P(x,y)$, $P(x)$ or $P(y)$? How do you compute the integral term?}



%\mh{\fref{re}: Replace A, B labels with \ref{f:re-a}, \ref{f:re-b}.}
%\mh{\fref{re}: In A, the two motions are should be time-aligned.}
%\mh{\fref{re}: In A, there is no need to plot the labels, as the colours show the same information.}
%\mh{\fref{re}: It would be good if both plots showed the \emph{same} sample movement.}
%\mh{\fref{re}: Figure titles are redundant: remove them.}
%\mh{\fref{re}: All axes must have units.}
%\mh{\fref{re}: Please convert $x$-axes to S.I. units (\ie seconds, \emph{not} time-steps).}
%\mh{\fref{re}: Please convert $y$-axis to S.I. units (\ie $ms^{-2}$ or $rad^{-2}$).}
%\mh{\fref{re}: Removed repeated/redundant information from legends.}
%\mh{\fref{re}: Ensure axes have the same scale.}
%\mh{\fref{re}: Use the caption to describe what is shown.}




%\mh{\done{I would expect a description of how the Support Vector Machine is trained, both for classification and regression, to appear here. What implementation do you use? What data is it given? What parameters are used? How do you avoid issues such as over-fitting? How many trials of learning are used? Why are these design choices justified?}}

%\mh{done{I would expect a description of what performance metrics you use and how they are computed to appear here. Why is measuring performance with these metrics appropriate?}}



%\subsection{Numerical simulation of centripetal acceleration and tangential acceleration for physical pendulum model}\label{s:simulation} 
%\mh{\done{If you do not report any results from experiments with data from the numerical simulation, \sref{simulation} should be omitted.}}

%\mh{\done{If you do not use any of the equations or quantities defined in \sref{physical_pendulum_model}, the section should be omitted.}}

%The time period of physical pendulum is given below. \cite{davidovits_physics_2019}
%\begin{equation}
%T = 2\pi\sqrt{\frac{I}{Wr}}
%\end{equation}

%where I is the moment of inertia of the pendulum, W is the total weight of the pendulum and r is the length of the pendulum.

%Equations of centripetal acceleration and tangent acceleration are shown respectively.\cite{davidovits_physics_2019}

%\begin{equation}
%\rddot_{y} = \frac{4\pi^2lsin(\theta)}{T^2}
%\end{equation}

%\begin{equation}
%\rddot_{z} = \frac{4\pi^2lcos(\theta)}{T^2}
%\end{equation}

%where $\theta$ is rotation angle.

%Finally, centripetal acceleration and tangent acceleration with respect to rotation angle and weight of pendulum can be obtained.

%\begin{equation}
%\rddot_{y} = \frac{sin(\theta)*L^{2}*w}{mr^2}
%\label{centripetal}
%\end{equation}

%\begin{equation}
%\rddot_{z} = \frac{cos(\theta)*L^{2}*w}{mr^2}
%\label{tangential}
%\end{equation}

%where $l$ is the distance of the center of gravity from the pivot point,  $r$ is the distance between the sensor to the rotation point, $m$ represents sensor of mass located a distance from the center of rotation and $w$ means the total weight of the pendulum.

\stepcounter{casestudy}%
\subsection{Case Study \thecasestudy: Human \acrlong{ar}}\label{s:human_ar}
The results from \sref{scotch_yoke} indicates that that sensors placed at loose positions of the fabric can provide a greater statistical distance, than that located in fixed positions. The increased statistical distance can contribute to the performance of \gls{ar}.

In this section, the role of motion artifact in a gesture recognition task is evaluated in a physical motion capture task.
\mh{\sref{human_ar} fine as far as it goes, assume will be properly written up!}%
\subsubsection{Material and methods}
To prove the finding from \sref{scotch_yoke} remains valid for human motion, this experiment uses \emph{hand winch} as a data acquisition device \footnote{The experiment reported here were conducted with the ethical approval of King's College London, UK : MRPP-21/22-33739.}. The participant who wears the loose shirt ($96\%$ cotton and $4\%$ spandex) rotate the \SI{15}{\cm} length crank handle with the guide of target point displayed on MATLAB interface. This interface plots two points in real time. Specifically, \il{\item red point represents the position of wrist-attached sensor and \item the tracking of blue point is uniform circular motion generated using} 
\begin{equation}
\vec{T(t)} =\vec{r}\sin(\w t) + \vec{r}\cos(\w t).
\end{equation}
where $T$ means the position of the target and $r = 130\si{\mm} $ is the radius of circle motion. From this, the participant should make sure that the two points are in the same place as far as possible in each trial. During this motion, one Aurora sensor is attached to a worn loose sleeve, at fixed positions. Anther Aurora sensor is placed securely on the wrist to act as a baseline. The experiment set up is shown in \fref{hand}\ref{f:hand-a}. With \emph{low} ($\w_{1} = 1.25\pi\si{\radian\per\second}$) and \emph{high} frequency ($\w_{2} = 2.5\pi\si{\radian\per\second}$) of the target point, hand can simply rotate crank handle with two different frequencies.  \id{maybe provide a short kinematic explanation of these?} With this set up, \NdhandExperiment\ sample trajectories of length $\Tk = \SI{8}{\second}$ at each frequency are recorded. In this duration, the first $\SI{3}{\second}$ is allowing the participant can follow the target properly. The rest of data are extracted for further analysis using the method described in \sref{scotch_yoke}.
\begin{figure}
\begin{tikzpicture}[ spy using outlines={blue,circle,magnification=4, size=1.2cm,connect spies}]
    % Use Wikipedias image of the day
    \node[anchor=south west,inner sep=0] (image) at (0,0){\includegraphics[width=0.5\linewidth]{figure/hand.pdf}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
     %   \foreach \x in {0,1,...,9} { \node [anchor=north] at (\x/10,0) {0.\x}; }
     %  \foreach \y in {0,1,...,9} { \node [anchor=east] at (0,\y/10) {0.\y}; }
        \end{scope}
    %\spy on ($0.95*(image.south east)+0.95*(image.north west)$) in node at ([xshift=0cm,yshift=-1cm]image.north);
    \spy on (4.05,0.6) in node at ([xshift=1.5cm,yshift=-0.7cm]image.north);
    \draw[stealth-,line width = 3pt,green] (3,2.1) -- (2.5,2.1) node[left,black,fill=white]{$\dr$};
    \draw[stealth-,line width = 3pt,green] (4.1,1.7) -- (4.1,1.1) node[left,black,fill=white]{$\df$};
    \draw[stealth-,line width = 3pt,green] (2.8,0.8) -- (2.8,0.3) node[left,black,fill=white]{Hand winch};
    \node at (0.5,0.5){\ref{f:hand-a}};
\end{tikzpicture}
\input{figure/hand_result}%
\caption{\cl{\item \label{f:hand-a} The participant rotates hand winch with wrist-attached sensor $\dr$ and cloth-attached sensor $\df$. \item \label{f:hand-b} Mean accuracy of \sref{human_ar} with $100$ trials ($\pm$ standard derivation) when varying window size.}}
    \label{f:hand}
\end{figure}
\subsubsection{Results}
\fref{hand}\ref{f:hand-b} shows the overall accuracy of \gls{ar} using the \gls{svm} classifier with different window sizes. The accuracy of cloth-attached sensor is higher at all window sizes. This is consistent with conclusions of \sref{sim} and \sref{scotch_yoke}.
\manuallabel{N_case_studies}{\numberstringnum{\thecasestudy}}% get number of case studies presented


==> data/problem_definition.tex <==
%\mh{\done{Use \sref{problem_definition} to define what problem the paper addresses in more precise terms than what is in \sref{introduction}. You should state any assumptions you make, and make precise what you mean by terms such as \gls{ar}, \gls{me}, \etc. It is an opportunity to set the scope of the work---\ie state what your paper addresses (and also what it \emph{does not} address).}}
The following introduces the proposed framework  and presents a worked example of its application to a simple movement classification task.
\subsection{Problem Definition}
\Acrlong{ar} is defined as the classification of movements into a number of discrete categories of activity (\eg sitting, standing, \etc) \id{\done{you keep using these examples, but are they relevant?}} based on motion data. For simplicity, in the following, it is assumed that the latter, $\Df$, consists of $\Nd$ measurements of the absolute position of a point $\pf$ on a garment, collected over an extended duration of time, at a regular sampling frequency. In \gls{ar}, each data point also contains a label\footnote{Throughout the paper, without loss of generality, the class labels are assumed to be binary.} $\y\in\{0,1\}$ corresponding to the category of movement, so $\DfAR=\{(\bxf_1,\y_1),...,(\bxf_\Nd,\y_\Nd)\}$. This is contrasted with so-called \emph{rigid data} $\Dr$, recorded under the same conditions, except that the sensor is rigidly attached to the moving body. The goal of \gls{ar} is to train a classifier on $\DfAR$ such that, when presented with (previously unseen) movement data $\bxfd$, the corresponding class label $\yd$ can be accurately predicted.

Previous studies have provided empirical evidence that, contrary to expectations, \gls{ar} performance is \emph{improved} when using data from \emph{loose fitting garments} \cite{michael2017}. This paper tests the hypothesis that this effect is due to \emph{artefacts} introduced by the motion of the fabric, thereby simplifying the task of distinguishing between movement categories. \id{this is really good}

\subsection{Probabilistic Model of Fabric Motion}\label{s:fabric_motion_model}
The effect of fabric motion on the data $\Df$ is subject to a high degree of uncertainty, arising from challenges in estimating the fabric's physical properties and the resultant movement complexity. To deal with this, it is proposed to model the data generation process through stochastic methods.

Specifically, the position $\bxf$ of the point $\pf$ on the fabric at any given time is modelled as the stochastic process consisting of the corresponding position $\bxr$ of a point $\pr$ on the rigid body plus a random offset $\bdelta$ introduced by the fabric motion.
In the univariate case, this can be written as
\begin{equation}
\Xf = \Xr + \Xd
	\label{e:Xf}
\end{equation}
where $\xf(t)\sim\Xf$, $\xr(t)\sim\Xr$ and $\delta(t)\sim\Xd$.

The key to determining whether the fabric movement is beneficial to \gls{ar} is to understand the effect of $\Xd$ on the statistical distance between movement classes. A condition for improved classification performance is a greater statistical distance in data distribution between movement classes in $\Df$ compared to $\Dr$, \ie
\begin{equation}
\Dd(\XfyO,\Xfyl) > \Dd(\XryO,\Xryl)
	\label{e:DXfXr}
\end{equation}
%\mh{It is not clear to me that \eref{DXfXr} is a \emph{necessary and sufficient} condition for better classification performance. Do you have any support for this? It seems to me that a counter example could be the following: Imagine you set the feature vector to consist of regular samples of the signal over a fixed duration. Two signals of different frequency, would occupy different parts of the feature space, enabling a decision boundary to be found that perfectly separates them. Is this not the case?}
%\mh{\done{By 'distribution' do you mean \gls{cdf}, \gls{pdf}, or does it not matter? The language here should be made as precise as possible.}}
where $\XfyO$ is the distribution of fabric data for movement class $\y=0$, $\Xfyl$ is the same for movement class $\y=1$, $\XryO$ and $\Xryl$ are the equivalent distributions for rigid data, and $\Dd(\cdot,\cdot)$ is a suitable metric in probability space. For the latter, several choices are available (\eg \gls{kl} divergence or \gls{js} divergence). 
%\mh{\done{This section is still describing the \emph{general} problem/approach, so descriptions/justifications in terms of the \emph{specific} example (mass/spring system) do not go here.}} 
In the following, the \gls{ks} metric is used \cite{justel1997multivariate}
\begin{equation}
	\begin{split}
&\Dd(\XfyO,\Xfyl)=\text{sup}\left| \FXfyO-\FXfyl\right|\\
&\Dd(\XryO,\Xryl)=\text{sup}\left| \FXryO-\FXryl\right|\\
	\end{split}
	\label{e:ks_def}
\end{equation}
where $\F(\cdot)$ denotes the \gls{cdf} \id{\done{Have you defined this?}} of a random variable. Note that, \gls{ks} is chosen since the range of possible fabric positions may differ depending on the movement, meaning that $\XfyO$ and $\Xfyl$ occupy different probability spaces, preventing measures such as \gls{kl} or \gls{js} from being computed.
%
In the next section, a simple worked example is presented to illustrate the effect of fabric motion on \acrlong{ar} predicted by this model.

\subsection{Example: Oscillatory Motion}\label{s:shm}
Consider the problem of movement analysis for a one dimensional, scotch yoke mechanism using data from a sensor mounted on an inextensible piece of fabric attached to the mechanism (see \fref{simulation}\ref{f:simulation-a}). Here, an \gls{ar} task might involve classifying a set movements of the rigid body (\eg those with different frequencies) from raw positional data.

\begin{figure}%
\input{figure/yoke.tex}%
\input{figure/position.tex}%
\caption{\cl{\item\label{f:simulation-a} A scotch yoke mechanism ($\phiy=0$) with a piece of fabric attached. Sensors are affixed at $\pr$ (the tip of the sliding yoke) and $\pf$ (the tip of the fabric). \item\label{f:simulation-b} Simulated signals of the sensors from this model ($\v\L = 0.3$).}}
\label{f:simulation}%
\end{figure}%
%\mh{\done{\fref{simulation}\ref{f:simulation-b}: Add units to the position }}
%\mh{\done{\fref{simulation}\ref{f:simulation-a}: Add an arrow to indicate the rotary movement of the wheel.}}
%\mh{\done{\fref{simulation}\ref{f:simulation-a}: Label the figure to define $\Ay$, $\w$ and $\phiy$.}}
\mh{\fref{simulation}\ref{f:simulation-a}: Label the figure to define $\phiy$.}
%\mh{\done{\fref{simulation}\ref{f:simulation-a}: Label the figure to define $\L$.}}
%\mh{\done{Please improve the quality of \fref{simulation}\ref{f:ma-a}. You could use a package like \texttt{tikz} for this. It would also help to label it with the symbols you use in the main text, \eg show $\xr$, $\xf$ \etc.}}
%\mh{\done{Be strict about your notation in \fref{simulation}. For instance, in \eref{Xf}, the symbol $\Xr$ denotes the \emph{random variable}, not the \emph{actual} position of the mass ($\xr(t)$), yet you use $\Xr$ in the diagram and in the legend.}}
%\mh{\done{\fref{simulation}: Please adjust the figure so that it fills the space (\ie avoid the wasted white-space).}}
%\mh{\done{\fref{simulation}: I don't understand what the `Reference point' is meant to represent.}}
%\mh{\done{\fref{simulation}: The attachment point of the fabric in this figure appears to be different to that show in \fref{mb}. This will cause confusion - please fix.}}
%\mh{\done{\fref{simulation}: Please add labels to points $\pr$ and $\pf$ for this problem.}}

In this system, the horizontal position of the rigid body (point $\pr$) over time is given by
\begin{equation}
\xr(t) =\Ay\sin(\w t+\phiy)
\label{e:xr}
%\label{mass:position}
\end{equation}
%\mh{\done{I've added the phase $\phiy$ to \eref{xr} - I assume this does not change the \gls{pdf} or \gls{cdf} of $\Xr$ or $\Xf$, correct?}}
where $\Ay$ is the amplitude%\mh{\done{I believe $\Ay$ is independent of the initial conditions for a Scotch Yoke.}}
, $\w$ is the frequency (equivalently, the angular speed of the rotary wheel of the mechanism) and $\phiy$ is the phase (equivalently, the starting angle of the wheel) and (without loss of generality) it is assumed $\Ay=1$. In this system, samples of the rigid body position follow a beta distribution
\begin{equation}
	\Xr\sim\B(\frac{1}{2},\frac{1}{2}).
	\label{e:Xr}
\end{equation}

As the rigid body moves, the fabric will move alongside it, but undergo additional motion due to the complex fabric dynamics according to \eref{Xf}. 
In general, the nature of the fabric motion will depend on \il{\item its physical properties (\eg mass distribution, stiffness, fibre structure, length, width, orientation) and \item the movement pattern of the rigid body (\eg amplitude, frequency)}. \edit{}{Noting that, here, the fabric is inextensible, the maximum possible displacement $\xd$ of the point $\pf$ from $\pr$ is $\L$, suggesting that a simple choice of its distribution could be}{mh}
\begin{equation}
\edit{}{\Xd\sim\U(-\L,\L).}{mh}
\end{equation}
\edit{}{However, this would imply that any displacement $-\L\le\xd\le\L$ is equally likely, whereas in practice, $\xd$ tends to be greater when there is greater excitation of the fabric by the movement of the yoke, \eg for higher-frequency movements. Therefore, the following assumes}{mh}
\begin{equation}
\edit{}{\Xd\sim\U(-\v\L,\v\L)}{mh}
\end{equation}
\edit{}{where}{mh}
\edit{The following focuses on the effect of the \emph{the sensor's position attached on the fabric $L$} and \emph{movement frequency} $\w$ since}{}{mh} \il{\item \edit{previous work has shown that fabric motion improves \gls{ar} of movements with different frequencies as $\L$ increases \cite{michael2017} and}{}{mh} \item \edit{the effect of these two factors is relatively simple to model for the oscillatory motions considered here}{}{mh}}. \edit{Specifically, at low frequency the movement of fabric is similar with}{}{mh} \id{\done{unclear to me?}} \edit{with the rigid body (see \fref{setup}\ref{f:setup-a}), whereas at high frequency there is greater excitation of the fabric  (see \fref{setup}\ref{f:setup-b}).}{}{mh} \id{\done{I think that figure 3 is unclear, black over black doe not help, have you tried plaing with the contrast?}} \edit{Moreover, the attachment point $\pf$ which is attached away from the tip of the fabric would collect the smaller range of possible position samples (see \fref{setup}\ref{f:setup-b}).}{}{mh} \id{\done{why is this relevant?}} \edit{Note that, as the fabric is inextensible, the maximum displacement $\delta$ of the point $\pf$ from $\pr$ when $\L$ is $1$.}{}{mh} %\mh{\done{\fref{mb} does not show the difference between fabrics of different lengths, but it should!.}}
%
\begin{figure}
\begin{overpic}
[width=0.5\linewidth]{figure/low.pdf}
\begin{tikzpicture}
\coordinate (ref) at (0,0);
\draw[decorate,decoration={brace,mirror,raise=8pt},ultra thick,white]  (ref)+(0.9,0.9) --  (2.7,0.9);
\node at (1.1,0.2)[right,fill=black,text=white,opacity=.25,text opacity=1]{Range of movement};
\filldraw[white] (ref)+(0.9,0.7) circle (2pt) node[anchor=west]{};
\filldraw[white] (2.7,0.7) circle (2pt) node[anchor=west]{};
\node at (0.3,0.2)[fill=black,text=white,opacity=.25,text opacity=1]{\ref{f:setup-a}};
\end{tikzpicture}
\end{overpic}
%\ref{f:setup-b}
\begin{overpic}
[width=0.5\linewidth]{figure/high.pdf}
\begin{tikzpicture}
\coordinate (ref) at (0,0);
\draw[decorate,decoration={brace,mirror,raise=8pt},ultra thick,white]  (ref)+(0.2,0.9) --  (3.4,0.9);
%\node at (0,0.2)[right,white]{Range of fabric position};
\node at (0.8,0.2)[right,fill=black,text=white,opacity=.25,text opacity=1]{Range of movement};
\filldraw[white] (ref)+(0.2,0.7) circle (2pt) node[anchor=west]{};
\filldraw[white] (3.4,0.7) circle (2pt) node[anchor=west]{};
\draw[decorate,decoration={brace,mirror,raise=8pt},ultra thick,white]  (ref)+(0.8,1.7) --  (2.8,1.7);
\node at (1.0,1)[right,fill=black,text=white,opacity=.25,text opacity=1]{Lower $\L$};
\filldraw[white] (0.8,1.5) circle (2pt) node[anchor=west]{};
\filldraw[white] (2.8,1.5) circle (2pt) node[anchor=west]{};
\node at (0.3,0.2)[fill=black,text=white,opacity=.25,text opacity=1]{\ref{f:setup-b}};
\end{tikzpicture}
\end{overpic}
%\ref{f:setup-c}
\input{figure/setup}
\caption{The scotch yoke mechanism with a piece of fabric attached \edit{is moving in}{moving at}{mh} \cl{\item \label{f:setup-a} low and \item \label{f:setup-b} high frequency. \item \label{f:setup-c} Front-view of the experiment set up.} Sensors are placed \il{\item at equidistant intervals along the fabric strip ($\df_{2}$-$\df_{4}$) and \item rigidly at the attachment point ($\dr_{1}$)}.}
\label{f:setup}
\end{figure}
\mh{\fref{setup}: Overlay (a), (b), (c) onto the photos.}
\mh{\fref{setup}: Make the bottom and top panels the same width.}
\mh{\fref{setup}: Minimise whitespace and maximise figure size.}
%\mh{\done{\fref{mh}: Improve the overall quality and appearance of this figure.}}
%\mh{\done{\fref{mh}: The green braces are nearly impossible to see.}}
%\mh{\done{\fref{mh}: Improve the labelling so that the effect of $\w$ and $\L$ become clearer.}}
%
%\mh{\done{This is the weakest part at the moment. You need to either show evidence either (i) from the literature or (ii) an experiment that this relationship between $\w$ and $\xf$ really exists.}}
%
\edit{Since the precise motion of the fabric is uncertain, $\delta$ is modelled to be uniform-randomly distributed $\Xd\sim\U(-\v\L,\v\L)$ where }{}{mh}
\begin{equation}
\edit{\v = 1-\exp(-(\w)^2).}{\v = 1-\exp(-\w^2).}{mh}
	\label{e:z}
\end{equation}
Note that, this respects the constraint that $-\L\le\delta\le\L$ (since \eref{z} causes $0\le\v\le1$) while capturing the tendency for $\delta$ to increase at higher frequencies \edit{}{up to a saturation point}{mh}.
%\mh{\done{Note that $-1\le\tanh(x)\le1$ so it seems \eref{z} is wrong.}}
%\mh{\done{Is \eref{z} correct? I think we agreed to use an equation with offset $\alpha$ and scaling $\beta$, something like $\v = \exp(-((\omega-\alpha)/\beta)^2)$.}}
%\mh{\done{Is \eref{z} correct? I think you mean $\v = 1-\exp(-(\w)^2)$.}}%
%\mh{\done{Does it matter what equation is used for $\v$? Does it change \ref{e:DXfXr} at all? If not, perhaps we can choose $\v$ according to the setup, so that differences in movement can go beyond differences in $\w$.}}
%\edit{We also assume the \gls{pdf} of additional information is uniform distribution ($Y\mathcal \sim {U}(-\v L,\v L)$), which indicates it can occur in this fixed range with equal probability. We also assume the maximum value of $\left|\v L\right| $ is $A$ ($0<\left|\v L\right| \leq A$) since the range of additional information would not be larger than the range of body movement in the real application.}{}{mh} \edit{We let $A = k = 1$ in the following computation.}{}{mh}

%With this model, the \gls{pdf} and \gls{cdf} of the mass position and the additional information are shown as below: 
%\begin{equation}
%f(X)=
%\begin{cases}
%\frac{1}{\pi\sqrt{1-X^2}}& \text{$-1<X<1$}\\
%0& \text{otherwise}\\
%\end{cases}
%\label{pdf:sine}
%\end{equation}

%\begin{equation}
%F(X)=
%\begin{cases}
%\frac{sin^{-1}(X)}{\pi}+\frac{1}{2}& \text{$-1<X<1$}\\
%0& \text{otherwise}\\
%\end{cases}
%\label{cdf:sine}
%\end{equation}

%The \gls{pdf} of the additional information is given by:

%\begin{equation}
%f(Y)=
%\begin{cases}
%\frac{1}{2\v L}& \text{$-\v L<Y<\v L$}\\
%0& \text{otherwise}\\
%\end{cases}
%\end{equation}


%(a)$\v L\geq 1$
%\begin{equation}
%f(T)=
%\begin{cases}
%\frac{sin^{-1}(T+\v L)+\frac{\pi}{2}}{2\v L \pi}& \text{$-1-\v L<T<1-\v L$}\\
%\frac{1}{2\v L}& \text{$1-\v L \leq T \leq -1+\v L$}\\
%\frac{sin^{-1}(-T+\v L)+\frac{\pi}{2}}{2\v L \pi}& \text{$-1+\v L<T<1+\v L$}\\
%0& \text{otherwise}\\
%\end{cases}
%\end{equation}

%(b)$0<\left|\v L\right|\leq 1$
%\begin{equation}
%f(T)=
%\begin{cases}
%\frac{sin^{-1}(T+\v L)+\frac{\pi}{2}}{2\v L \pi}& \text{$-1-\v L\leq T <-1+\v L$}\\
%\frac{sin^{-1}(T+\v L)-sin^{-1}(T-\v L)}{2\v L \pi}& \text{$-1+ \v L \leq  T \leq 1-\v L$}\\
%\frac{sin^{-1}(-T+\v L)+\frac{\pi}{2}}{2\v L \pi}& \text{$1-\v L < T \leq \v L+1$
%}\\
%0& \text{otherwise}\\
%\end{cases}
%\end{equation}
According to this model, the \gls{cdf} of $\Xr$ is \cite{shin2008fundamentals} 
\begin{equation}
F(\xr)=
\begin{cases}
	\frac{\sin^{-1}(\xr)}{\pi}+\frac{1}{2} &-1\leq \xr \leq 1\\
0& \text{otherwise}\\
\end{cases}
\label{e:cdf:sine}
\end{equation}
and it can be shown\footnote{A derivation is provided in \sref{pdf},  \sref{cdf}.} that the \gls{cdf} of $\Xf$ is
%\providecommand{\vp}{\v_+}%
%\providecommand{\vm}{\v_-}%
\begin{equation}
	F(\xf)=
	\begin{cases}
		0        &            \xf<-1-\v\L\\
		F_1(\xf) & -1-\v\L\leq\xf<-1+\v\L\\
		F_2(\xf) & -1+\v\L\leq\xf\leq 1-\v\L\\
		F_3(\xf) &     1-\v\L<\xf\leq\v\L+1\\
		1        &            \xf>1+\v\L 
	\end{cases}
	\label{e:CDFXf}
\end{equation}
where %
\begin{equation}
	F_1(\xf)=\frac{\pi\vp+2\sqrt{1-\vp^2}+2\vp\sin^{-1}\vp}{4\v\L\pi},%
\end{equation}%
\begin{equation}%
\begin{split}%
	F_2(\xf)&=\frac{1}{2}+\\&\frac{\sqrt{1-\vp^2}-\sqrt{1-\vm^2}+\vp\sin^{-1}\vp-\vm\sin^{-1}\vm}{2\v\L\pi},\\%
\end{split}%
\end{equation}%
\begin{equation}%
\begin{split}%
F_3(\xf)=\frac{\frac{3 \pi \v L + \pi \xf}{2}-\vm sin^{-1}(\vm)-\sqrt{1-\vm^2}}{2\v L \pi}\\
\end{split}%
\end{equation}%
and $\v_\pm=\v\L\pm\xf$. The \gls{pdf} and \gls{cdf} of $\Xr$ and $\Xf$ are shown in \fref{pro}\ref{f:pdf} and \ref{f:cdf}, respectively. As can be seen in \fref{pro}\ref{f:pdf},\id{\done{grammar}} the range of fabric positions is larger than that of the rigid body, meaning they occupy different probability spaces.
%\mh{\done{Explain what the significance of \eref{cdf:sine} and \eref{CDFXf} is. What are the important features of these equations?}}%
%\mh{\done{It is not clear what \fref{pro} is meant to show.}}

\begin{figure}%
\input{figure/pdf}%
\input{figure/cdf}%
\caption{The \cl{\item\label{f:pdf} \gls{pdf}  and \item\label{f:cdf} \gls{cdf} of rigid body and fabric position ($\v\L = 1$).}}%
\label{f:pro}%
\end{figure}%
%\mh{\done{Are you sure the lines are correctly labeled in \fref{pro}? In \fref{pro}\ref{f:pdf} the \color{red}{red} line looks like the arcsin distribution, so I would expect it to be the curve for the mass (\ie $\Xr$), but it is labelled as $\Xf$. In \fref{pro}\ref{f:cdf} the \textcolor{blue}{blue} line looks like the \gls{cdf} of the arcsin distribution, but it is labelled as $\Xf$.}}
%\mh{\done{\fref{pro}: Are the dashed lines in \fref{pro}\ref{f:pdf} meant to be there? What do they represent?}}
%\mh{\done{\fref{pro}: The label for the $x$-axis is missing.}}
From \eref{cdf:sine} it is apparent that the \gls{cdf} of $\Xr$ is \emph{independent of $\w$}, meaning that if the \gls{ar} task is to classify movements of different frequency (\eg $\w_1$ and $\w_2$) \emph{the data distribution can not increase statistical distance to discriminate between classes}, \ie $\Dd(\Xr_{\w_1},\Xr_{\w_2})%=\Dd(\Xr_{\y=0},\Xr_{\y=1})
=0$. However, from \eref{CDFXf}, it can be shown that \footnote{A derivation is provided in \sref{fabric}.}
\begin{equation}
	\begin{split}
\Dd(\Xf_{\w_1},\Xf_{\w_2}) &= \text{sup}\left| F(\Xf_{\w_1})-F(\Xf_{\w_2})\right|\\
&=\left| F(\xf_{\w_1|\xf=1+\v_{1}L})-F(\xf_{\w_2|\xf=1+\v_{1}L})\right|\\
&=\frac{\pi (\dv L - 1) +2\sqrt{1-(\dv L- 1)^2}}{4\v_{2} L \pi}\\
&-\frac{ 2(1 -\dv L)sin^{-1}(\dv L -1 )}{4\v_{2} L \pi}
		\label{e:ks:classification}
	\end{split}
\end{equation}
where $\dv = |\v_{2} - \v_{1}|$.
%\mh{\done{You need to define a different symbol here! How about $\dv$? Please amend \eref{ks:classification} accordingly (\ie make clear what is $\v$ and what is $\v_{12}$).}}
%\mh{\done{Make \eref{ks:classification} more compact.}}
As $\Dd(\Xf_{\w_1},\Xf_{\w_2})>0$ the condition \eref{DXfXr} is met, suggesting that \emph{\gls{ar} based on the motion of the fabric} will lead to \emph{higher classification performance}.

Moreover, it can be shown that \emph{$\Dd(\Xf_{\w_1},\Xf_{\w_2})$ increases with $\L$ or $|\w_{2}-\w_{1}|$}, suggesting that \il{\item  \emph{the looser \edit{of}{}{mh} the fabric, the greater \edit{}{the }{mh}statistical distance}\footnote{A proof is provided in \sref{increase}.} and \item \emph{the bigger \edit{}{the }{mh}difference between two movement \edit{frequency}{frequencies}{mh}, the greater \edit{}{the }{mh}statistical distance}\edit{}{.}{mh}\footnote{A proof is provided in \sref{fre}.}} An empirical study of this example is provided in the next section.

%\mh{\done{The argument presented in \sref{shm} seems a bit circular. You first introduce frequency dependency into the fabric data, and then state that this means that fabric data is better for classifying movements of different frequency.}}
%\mh{At this point, the focus should switch back to the general problem.}fre

%\subsubsection{Methods}
%\edit{We employ \il{\item \gls{ks} to measure probability distribution similarity and \item \gls{svm} as machine learning algorithm to solve task of \gls{ar} and \gls{me}.} In terms of \gls{ks}, it computes the maximum difference $D$ between \gls{cdf} of two measurements followed by the definition of \gls{ks} \cite{ghasemi2012normality}. For \gls{svm}, simulated dataset consists of train data and test data. We combine all n-th odd numbers of simulated dataset as train data and all n-th odd numbers of simulated data as test data. We use \gls{rbf} as kernel function. \gls{svm} is implemented by the Libsvm toolbox \cite{chang_libsvm_2011} and MATLAB R2020b (MathWorks, USA). It also repeats $100$ times to ensure the robustness of the result. The \gls{svm} setting for both tasks in this simulation are consistent. To the end, we compute \gls{pcc} between accuracy of \gls{ar} or \gls{me} evaluated by \gls{svm} and the maximum difference from \gls{ks} to investigate whether it is possible to predict performance of \gls{svm} from \gls{ks}.}{}{mh}

%\subsubsection{\Acrlong{ar}}
%\edit{In \gls{ar}, it is to perform classification between two motions with frequency ($\w_{1}=1,\w_{2}=2$) using two different weights of the mass ($m_{1}=1,m_{2}=\frac{1}{4}$). Different frequency of mass movement could have influence on the range of additional information as described before. Therefore, we compute $\v$ from equation (\ref{z}) to get $\v_{1}=1$ and $\v_{2}=\frac{1}{\mathrm{e^{4}}}$.}{}{mh}

%\edit{Given the movement at the duration of $t$ ($ t =2\pi$) using two different weights of the mass, we generate mass position ($X_{1},X_{2}$) from equation (\ref{mass:position}) at \SI{100}{\Hz}. This can get $N = 100 \times 2\pi \approx 629$ data points to form matrix $X_{1}^{629 \times 1}$ and $X_{2}^{629 \times 1}$. To simulate fabric position, equation (\ref{fabric:position}) is used to form matrix $T_{1}^{629 \times 1}$ and $T_{2}^{629 \times 1}$.}{}{mh}

%\edit{In \gls{ks}, equation (\ref{cdf:sine}) shows the \gls{cdf} of sine wave is irrelevant to the mass weight and its frequency. Therefore, the maximum difference ($D$) between \gls{cdf} of mass position with two frequency $\w_{1}$ and $\w_{2}$ is $0$ ($D_{X_{1},X_{2}}=0$). As such, we get equation (\ref{ks:classification}) to compute the maximum difference ($D_{T_{1},T_{2}}$) from \gls{ks} on the position of the fabric ($T_{1},T_{2}$). }{}{mh}
%\begin{equation}
%\begin{split}
%&\edit{D_{T_{1},T_{2}}\mathop{=}\limits_{\text{sup}} \left| F(T_{1})-F(T_{2})\right|}{}{mh}\\
%&\edit{=1}{}{mh}\\
%&\edit{-(\frac{\frac{3\pi L + \pi (1+\frac{1}{\mathrm{e}^4}L)}{2} +2\sqrt{-( L-1) L}-\sqrt{-(2 %L-1)^2+1}}{2 L \pi}}{}{mh}\\
%&\edit{+\frac{(1+\frac{L}{\mathrm{e}^4}- L)sin^{-1}( L-1-\frac{L}{\mathrm{e}^4})-\sqrt{- (L-1-\frac{L}{\mathrm{e}^4})^2+1}}{2 L \pi})}{}{mh}\\
%\label{ks:classification}
%\end{split}
%\end{equation}

%\begin{figure}
%\begin{overpic}
%[height=0.4\linewidth]{svm_ar.eps}
%\put(0,0)
%{\ref{f:simulation:ar-a}}
%\end{overpic}~%
%\begin{overpic}
%[height=0.4\linewidth]{ks_ar.eps}  
%\put(8,0)
%{\ref{f:simulation:ar-b}}
%\end{overpic}%
%\caption{\cl{\item\label{f:simulation:ar-a} \edit{The \gls{ar} result of \gls{svm} based on simulated data.}{Accuracy of \gls{ar} using \gls{svm} classifier trained on fabric data against fabric length (mean$\pm$s.d. over \TrialsscotchYokeSimulation\ trials).}{mh} \item\label{f:simulation:ar-b} \edit{The result of $D$ computed from equation (\ref{ks:classification}).}{$\Dd(\Xf_{\w_1},\Xf_{\w_2})$ with varying $\L$ computed from \eref{ks:classification}.}{mh}}}
%\label{f:simulation:ar}
%\end{figure}
%\mh{I suggest you plot \fref{simulation:ar}\ref{f:simulation:ar-b} with \texttt{tikz} similar to how you did for \fref{pro}, to make the style consistent and to ensure the correct symbols are used.}
%\mh{Perhaps \fref{simulation:ar}\ref{f:simulation:ar-a} and \ref{f:simulation:ar-b} could be overlaid on the same axes.}
%\mh{Please improve the quality of \fref{simulation:ar}\ref{f:simulation:ar-a}. The axis label should not be longer than the axis. Perhaps you can use \texttt{tikz} to plot this data to improve the rendering.}
%\mh{Please add a line to \fref{simulation:ar}\ref{f:simulation:ar-a} for accuracy trained on rigid body data.}


%\edit{Fig. \ref{f:simulation:ar}\ref{f:ma-a} and \ref{f:ma-b} describe \gls{ar} accuracy from \gls{svm} and the maximum difference from \gls{ks} respectively. This result reveals longer length of fabric ($L$) can make more diverse on two distributions of data. Moreover, this dissimilar can improve \gls{ar} result. On the other hand, the accuracy of \gls{ar} from \gls{svm} on the mass position ($X_{1},X_{2}$) is $50\%$, which indicates the worst performance and has no ability to perform \gls{ar}. This tells classification on two class of data with the same distribution is an extremely challenging task.}{}{mh}

%\edit{The correlation coefficients between classification accuracy and $D_{T_{1},T_{2}}$ is $0.9718$, which reveals that two results have very strong positive correlation so that it is possible to predict classification accuracy from ks test.}{}{mh}

%\subsubsection{\Acrlong{me}}
%\mh{For the time being, I suggest that we focus the discussion on \gls{ar} in this paper, and omit the parts about \gls{me} until we can come up with a more positive message about it. (This could, for example, be around positioning sensors on the body.)}
%\edit{The problem of \gls{me} is to estimate mass position ($X$) giving fabric position ($T$). We assume it uses mass ($m_{1}=1$). In this case, we use $T_{1}^{629 \times 1}$ to estimate $X_{1}^{629 \times 1}$. As such, the maximum difference ($D_{T_{1},X_{1}}$) between \gls{cdf} of mass position and fabric position is given by:}{}{mh}
%\begin{equation}
%\begin{split}
%&D_{T_{1},X_{1}}\mathop{=}\limits_{\text{sup}} \left| F(T_{1})-F(X_{1})\right|=1\\
%&-(\frac{2\sqrt{-(L-1) L}-\sqrt{-(2L-1)^2+1}}{2L \pi}\\
%&+\frac{-\sqrt{-(L-1)^2+1}+(1-L)sin^{-1}(L-1)+\frac{3\pi L + \pi}{2} }{2L \pi})\\
%\label{ks:regression}
%\end{split}
%\end{equation}


%\edit{The relationship between fabric length $L$ and $D_{T_{1},X_{1}}$ can be seen in Fig. \ref{f:ma}\ref{f:ma-b}. From this, it is known that $D_{T_{1},X_{1}}$ is increasing when fabric length $L$ is raising. Fig. \ref{f:ma}\ref{f:ma-a} shows \gls{mse} of the estimation when fabric length ($L$) is increasing. %\mh{\done{I suggest you express this in terms of $\lim_{l\rightarrow\infty}KL(X||T)$.}} 
%which predicts that longer fabric length $L$ gradually
%\mh{From Fig.~\ref{simulation}(a) it looks like $\lim_{l\rightarrow\infty}KL(P||Q)=c$ where $c$ is some constant, which contradicts this argument.}
%}{}{mh}

%\edit{From this, the amount of additional information is larger with longer fabric length. This cause more serious information loss about target to make \gls{me} more difficult. }{}{mh}

%\edit{The correlation coefficients between \gls{mse} and $D_{T_{1},X_{1}}$ is $0.9163$, which reveals that two results also have very strong positive correlation so that it is possible to predict performance of \gls{me} from ks test.}{}{mh}

%
%\subsection{Statistical Learning Methods}
%\edit{Following the above simulation, this paper will evaluate this hypothesis in the real world. Pendulum is chosen to simulate shank movement as physical model since the rotation center of shank movement is knee and swinging motion of the pendulum is also pivoted at the center of circle \cite{davidovits_physics_2019}. A piece of fabric is attached on the pendulum is simulated as the cloth worn on the user. To simulate more complicated and natural patterns of shank movement, this pendulum also can swing bi-directional at different setting speeds using a DC motor.}{}{mh} 
%
%\edit{Motion analysis might need to use readings \texttt{$\y\in\R^p$} from the sensor $F$ which mounted on an item of clothing (\ie trouser). }{}{mh}
%\mh{\done{In the kinds of problems we're interested in, typically, we will \emph{only have data from fabric mounted sensors} (\ie no body-mounted sensor data). We are trying to \emph{avoid} the need for body mounted sensors for various reasons (comfort, usability, \etc). In the experiments described in this paper you have body-mounted sensors to be able to investigate the problem, but these will be absent in the end application. So you need to re-work this argument.}} 
%\mh{\done{Please avoid using raw \LaTeX\ for symbols. Use/make definitions in \texttt{tex/symbols.tex} instead. This makes it easier to change them if needed, and ensure mathematical consistency.}}
%\mh{\done{A more standard notation is to use the symbol $y$ for observations (\ie sensor readings), and $\phi$ for features derived from the raw readings.}} 
%\edit{In this, readings \texttt{$\bm{y}$} can form matrix $\bm{y}:=(y_{1},y_{2},..,y_{p})^\mathrm{T}$ and $y_{t}$ is the sensed reading at time $t$.}{}{mh}
%\mh{Use bold symbols to represent vectors.}
%\mh{\done{It is unclear why this is a vector. In other words, what does each element represent? A sample in time? An IID sample? The signal from a channel?}} 
%\edit{To have a reference to present how additional information affects \gls{ar} and \gls{me}, we also use sensor $R$ which located rigidly on the shank used as benchmark. }{}{mh}
%
%\edit{This paper uses \gls{svm} as supervised learning to solve problem of \gls{ar} and \gls{me}. This is also a dominant approach in wearable sensing systems \cite{cortes1995support}. On the other hand, we also compute \gls{js} to show the similarity of two different motions in \gls{ar} and \gls{js} between rigid-pendulum motion and fabric-attached motion in \gls{me}. These similarity can explain the results achieved from \gls{svm} and it also can be used to predict performance of \gls{ar} and \gls{me}. The following conceptual flow diagram describes the link between tasks, approaches and data. }{}{mh}
%
%\mh{\done{Perhaps you can create a conceptual flow diagram, showing the link between fabric-mounted sensors, information theory, and \gls{ar}/\gls{me}.}}
%
%\begin{figure}[htbp]
%\centerline{\includegraphics[height=0.8\linewidth]{concept.eps}}
%\caption{This is a concept flow diagram to show the relationship between tasks, approaches and data in this paper.}
%\label{f:concept}
%\end{figure}
%\mh{Remove \fref{concept}.}


==> figure/ks.tex <==
\begin{center}
\begin{tabular}{*{5}{|c}|} 
 \hline
 Sensor & $\dr_{1}$ & $\df_{2}$ & $\df_{3}$ &$\df_{4}$\\ [0.5ex] 
 \hline
 $\Dd$ & $0.04 \pm 0.004$& $0.1\pm 0.008$& $0.2\pm 0.001$  & $0.28\pm 0.02$\\%  [1ex] 
 \hline
\end{tabular}
\end{center}


==> figure/low.tex <==
\usetikzlibrary{calc}
\begin{tikzpicture}
    \node (image) at (0,0) {
        \includegraphics[scale=0.3]{low.pdf}
    };

\end{tikzpicture}

==> human_analysis.tex <==
\subsection{Set up}
The results from the simulation indicate that sensor positioning and motion speed place key roles in swing pendulum motion analysis. It is also seen, that motion artifact can increase classification accuracy but get regression more challenging.   




In this section, the role of motion artifact is investigated in a real human motion. For this, one participant performed similar visually walking and running. During this time, the participant is wearing tight pants and soft pants, which means parameter of length in pendulum experiment. Two tri-axis accelerators were attached on body and cloth and simultaneously recording acceleration. Using walking and running is corresponding to two different swing speeds generated by non-weighted pendulum and weighted pendulum.

\subsection{Motion recognition result}

\subsection{Motion estimation result}

==> mass_spring.tex <==
\usetikzlibrary{patterns}%
\begin{tikzpicture}
% Supporting structure
\fill [pattern = north west lines] (-1.5,0) rectangle ++(3,.2);%
\draw[thick] (-1.5,0) -- ++(3,0);%
% Spring 
\draw
[
    decoration={
        coil,
        aspect=0.3, 
        segment length=1.2mm, 
        amplitude=2mm, 
        pre length=1mm,
        post length=1mm},
    decorate
] (0,0) -- ++(0,-2) 
 node[midway,right=0.25cm,black]{$k$};%
% Mass
\node[draw,
    fill=blue!100,
    minimum width=1cm,
    minimum height=0.75cm,
    anchor=north,
    label=east:$\Xr$] at (0,-2) {};%
% fabric
\draw [fill=red, thick] plot [smooth,tension=0.5] 
coordinates {(0,-2.75)(-0.25,-2.75) (-0.25,-4) (0,-3.75) (0.25,-4) (0.25,-2.75)(0,-2.75)};%
\node at (0.75,-3.35){$\Xf$};%
\node at (-1.25,-3.9){\ref{f:ma-a}};%
\end{tikzpicture}

==> methods.tex <==
%\mh{\sref{background} needs to be linked to the preceding section. Give a more specific and in-depth discussion of the issue you are addressing, and why it's important. State the ways that others have approached it. Explain your approach, and why it is a contribution beyond the state of the art.}

%\subsection{Mutual information}\label{s:mutual_information}
%\mh{\sref{mutual_information} needs to be connected to the rest of the paper. As a reader, it is unclear why you are suddenly discussing \gls{mi}.}
%\Gls{mi} is an approach to tell the degree of difficulty to know the variable from the other variable, it also can be thought as the reduction of uncertainty of knowing about one variable, when another is given \cite{cover_elements_2012}.\mh{Rephrase.}\id{I think that I know what you mean, but I suggest to clarify these initial sentences}

%Formally, the \acrlong{mi} for two variables $X$ and $Y$ is given as \cite{cover_elements_2012}\edit{.}{}{mh} 
%\begin{equation}
%I(X;Y) = H(X)+H(Y)-H(X,Y)
%\label{mi}
%\end{equation}
%\mh{Symbols that have not been defined or explained: $X,Y,\mathcal{Y},\mathcal{X}$.}
%where $H(X)$, $H(Y)$ denote the entropy of $X$ and $Y$, and $H(X,Y)$  is their joint entropy. The calculation of entropy and joint entropy are shown in equation \eqref{entropy} and equation \eqref{joint_entropy}.
%\mh{What is the intuitive meaning of \eref{mi}? Can you explain why it takes this form?}

%\begin{equation}
%H(X)=-\sum_{i=1}^{n}P(X_{i})log_{2}P{(X_{i}})
%\label{entropy}
%\end{equation}

%\begin{equation}
%H(X,Y)=-\sum_{i=1}^{n}\sum_{j=1}^{n}P(X_{i},Y_{j})log_{2}[P(X_{i},Y_{j})]
%\label{joint_entropy}
%\end{equation}
%Where $P(X)$, $P(Y)$ denote the marginal probabilities of $X$ and $Y$, and $P(X,Y)$ denotes the joint probability.

%This concept can be used in classification and regression.\mh{From here...} \edit{Activity recognition}{\Gls{ar}}{mh} (\edit{}{\ie}{mh} classification) aims to automatically classify movements into a number of activities (\eg running, walking) when class data is provided. The more reduced uncertainty of label prediction means better classification performance while less reduced uncertainty shows worse classification accuracy. 

%In \edit{motion estimation}{\gls{me}}{mh} (\edit{}{\ie}{mh} regression), human motion measurement (\eg gait kinematics, walking/running speed) can be seen as label, in experiments, actual human motion is collected from body-attached sensor due to they are rigidly attached while cloth-attached sensor measurement contains motion artifacts so it uses cloth-attached sensor measurement to regress body-attached sensor measurement. Low mutual information tells that it is challenge to predict human motion when cloth-attached sensors measurement is known while high mutual information shows it is simple to notice human motion from cloth-attached sensors measurement. 
%\mh{... to here has nothing to do with \gls{mi}: it is a discussion about behaviour analysis.} \id{this whole section is extremely confusing. I think that you need to limit the explanation of the theory that is well established and focus more on your specific application}

%Therefore, a hypothesis that mutual information should be positively corresponding to classification accuracy and inversely proportional with mean squared error in regression is proposed.\mh{If this is the main way to measure the use of the \gls{mi}, then showing this correlation for several different classification and regression approaches would strengthen your argument.}

%Correlation coefficient (\eg\gls{pcc}) is anther method to find the relationship between two variables.\mh{It is unclear why you include this paragraph. Will you use this?} The main difference with \gls{mi} measures the general dependence while \gls{pcc} only can measure the linear dependence. \cite{clavier_mutual_2009}\mh{Broken reference.} Therefore, \gls{pcc} is not well suited to the task of human motion analysis. The reason is there is no linear relationship between class data and class label (see Fig.~\ref{re}(A)). Moreover, \gls{mi} is a more general method, more widely to be used and it can handle more complicated data or situation. But, the advantage of \gls{pcc} is simpler and more sufficient \cite{li_mutual_1990}.\mh{Broken reference.} 
%\mh{\done{What other measures could you use? Why do you choose \gls{mi} instead of those measures?}}
%\mh{Did you take a look at \textcite{Reshef2011}?}
%\mh{\done{The preceding two paragraphs need rewriting to make them clearer. It would be better to describe in general terms first, then go to the specific problems your paper considers. For instance, ``\Gls{mi} quantifies how much knowing one random variable (\eg $X$) tells us about the other (\eg $Y$) --see, \eg \textcite{murphy_machine_2012}. In the cases considered here, the random variables represent the sensor reading and the quantity of interest (activity in classification, or motion feature in regression).''}}
%\mh{The whole of \sref{background} needs rewriting to make it clearer. The text should follow a logical sequence, gradually building up your arguments. At the moment, this section reads like a random collection of ideas, but it is not clear what ties everything together. I suggest describing the problem in general terms first, then going into the specifics.}

This experiment uses simple pendulum model attached with a piece of fabric to investigate how amount of addition information contained in sensor measurement can effect performance of \gls{ar} and \gls{me}. 


\subsection{Information theory}\label{s:information_theory}
\subsubsection{Entropy}\label{s:entropy}
The entropy of a random variable is the average level of uncertainty inherent in the variable's possible outcomes. Considering the event $Q$\mh{You should relate this to the problem you are addressing. What is $Q$ in your problem? The reading from $\sensorR$ or $\sensorF$? Are these discrete or continuous-valued?} has possible outcomes $x_{1},...x_{n}$ with \edit{possibility of}{probability}{mh} $\Prob{P}{(x_{1})},...\Prob{P}{(x_{n})}$, the entropy of event $Q$ can be computed as \eqref{e:entropy} \cite{shannon1948mathematical}.\mh{\eref{entropy} is the entropy for a \emph{continuous-valued} random variable, whereas the text describes a \emph{discrete} set of outcomes. Which is correct?}
\begin{equation}
H(Q)=-\int_{i=1}^{n} \Prob{P}(x_{i})log_{2}\Prob{P}(x_{i})\,d(x)\edit{}{.}{mh}
\label{e:entropy}
\end{equation}
\mh{The integration limits in \eref{entropy} don't make sense.}

%\begin{equation}
%H(x_{i}) = -\sum_{i=1}^{n}\sum_{i=1}^{i} \alpha_i\frac{1}{\sqrt{|\Sigma_i|(2\pi)^d}}\exp(-\frac{1}{2}(x-\mu_i)\Sigma^{-1}(x-\mu_i)\top)\log_{2}{\alpha_i\frac{1}{\sqrt{|\Sigma_i|(2\pi)^d}}\exp(-\frac{1}{2}(x-\mu_i)\Sigma^{-1}(x-\mu_i)\top)}
%\label{entropy_gmm}
%\end{equation}

%\subsubsection{\gls{em} algorithm for \gls{gmm}}\label{s:em}
\subsubsection{\Acrlong{em} algorithm for \acrlong{gmm}}\label{s:em}
\mh{Again, you need relate this to the problem you are addressing. Why do you need to do \gls{em}? Why are you trying to fit a \gls{gmm}?}
\edit{\gls{gmm} consists of several Gaussian distributions.}{}{mh} The \edit{Gaussian density}{\gls{gmm} \gls{pdf}}{mh} can be expressed \edit{by equation \eqref{e:gmm}}{as}{mh} \cite{lan2006estimating}\edit{.}{}{mh}
\begin{equation}\label{e:gmm}
p(x) = \sum_{i=1}^{i} \omega_{i} G_i(x)
\end{equation}\mh{Upper limit of the sum in \eref{gmm} should not be $i$.}
\edit{Where}{where}{mh} $G_i(x)$ is the \gls{pdf} of \edit{each}{the $i$th}{mh} Gaussian component, \edit{$\omega$}{$\omega_i$}{mh} is the weight\edit{s}{}{mh} for the corresponding component, \edit{}{and}{mh} $\sum_{i=1}^{i} \omega_{i} =1$\edit{ and $i$ is the number of single Gaussian in \gls{gmm}}{}{mh}.

\edit{\gls{em} algorithm is an iteration method to maximum likelihood estimation, which is used to estimate parameters of Gaussian distribution and split \gls{gmm}}{The \gls{em} algorithm is used to fit the parameters of the \gls{gmm}}{mh} \cite{mclachlan2004algorithm}.

\subsubsection{Entropy of the \gls{gmm}}\label{s:entropy_gmm}
\mh{Again, you need relate this to the problem you are addressing. Where does multivariate modelling come in? Is your data multivariate? How/why?}
The \gls{pdf} of \edit{}{a}{mh} multivariate Gaussian distribution is \edit{know as equation \eqref{pdf}}{}{mh} \cite{cover_elements_2012}\edit{.}{}{mh}

\begin{equation}
p(x|\mu,\Sigma) = \frac{1}{\sqrt{|\Sigma|(2\pi)^d}}\exp(-\frac{1}{2}(x-\mu)\Sigma^{-1}(x-\mu)^\mathrm{T})\edit{}{.}{mh}
\label{e:pdf} 
\end{equation}
Referring \edit{from}{to}{mh} equation \eqref{e:entropy}\edit{}{,}{mh} \eqref{e:gmm} and \eqref{e:pdf}, the entropy of \gls{gmm} can be computed.\mh{Do not confuse the \emph{multivariate  Gaussian} with the \emph{\gls{gmm}}. A multivariate Gaussian allows multi-dimensional random variables to be captured in a \emph{single-component Gaussian \gls{pdf}}. A \gls{gmm} uses multiple Gaussian components to approximate an arbitrarily complex \gls{pdf}. The latter can be univariate, or multivariate.}

\subsubsection{\gls{kl}}\label{s:kl}
\edit{}{The}{mh} \acrlong{kl}, also known as relative entropy, is a measure of the asymmetry of the difference between two probability distributions. \edit{$KL(P||Q) \neq KL(Q||P)$.}{}{mh} In information theory, \gls{kl} is equivalent to the difference between entropy of two probability distributions \cite{nielsen2020generalization}. Suppose that $P(x)$ and $Q(x)$\mh{Conflicting notation: in \sref{entropy} $Q$ is an event, but here it is a \gls{pdf}.} are two probability distributions on two random variables, then in the continuous case, the \edit{definitions of \gls{kl} are:}{definition of \gls{kl} is}{mh} \cite{nielsen2020generalization}
\begin{equation}
KL(P||Q) = \int_{i=1}^{n} P(x_{i})log\frac{P(x_{i})}{Q(x_{i})}\,d(x)\edit{}{.}{mh}
\label{e:kl} 
\end{equation}
\mh{The integration limits in \eref{kl} don't make sense.}
The value of \gls{kl} is non-negative\edit{. It is increasing with unbonded when difference between the entropy of two probability distributions is rising, which can be shown as: $KL(P||Q):\geq 0$ }{}{mh}\cite{nielsen2020generalization}.

\subsubsection{\gls{js} in \gls{ar} and \gls{me}}\label{s:js}
\Acrlong{js} is based on a variant of \gls{kl}, it solves the problem of asymmetry of \gls{kl} \cite{nielsen2020generalization}.
\begin{equation}
JS(P\edit{:}{||}{mh}Q) = \frac{1}{2}KL(P||M) +  \frac{1}{2}KL(Q||M)
\label{e:js} 
\end{equation}\mh{Be consistent in notation. Avoid switching between use of $,$, $||$ and $:$.}
\edit{Where}{where}{mh} $M = \frac{P+Q}{2} $.
\gls{js} measures the similarity of two probability distributions ($P$ and $Q$). \edit{It is defined as \cite{nielsen2020generalization}.}{It can also be expressed as}{mh}
\begin{equation}
JS(P\edit{:}{||}{mh}Q) = H\left(\frac{P+Q}{2}\right) - \frac{H(P)+H(Q)}{2}
\label{js} 
\end{equation}

Generally, the \gls{js} is symmetric $JS(P:Q) = JS(Q:P)$, and its value is strictly \edit{bonded}{bounded}{mh} between $0$ and $1$ if using the base $2$ logarithm in the computation. $0 \leq JS(P:Q)\leq 1$ \cite{nielsen2020generalization}. This property \highlight{matches}{mh} with classification accuracy ($[0\%,100\%]$) in \gls{ar} and R-squared\mh{Notation conflict: $R$ is previously used to denote the rigidly-attached sensor.} ($[0,1]$) in \gls{me}.\mh{What is the precise meaning of \emph{matches} here? Can you formally show a relationship? Or is it just analogous?}

The \gls{js} is zero only if $P(x)$ and $Q(x)$ are completely the same. While it gets one when they are thoroughly different.

In the task of \gls{ar}, $P(x)$ and $Q(x)$ \edit{donate}{denote}{mh} two data distributions collected from similar activities (\eg walking and running). Higher \gls{js} refers to different data distributions between two classes, which expect to achieve higher classification accuracy. 

In the task of \gls{me}, it uses $Q$ as approximate distribution model (\eg cloth movement) to estimate the target $P$ (\eg actual human movement). Higher \gls{js} represents different data distributions between target and data means poor estimation performance (lower R-squared ($R^{2}$)).\mh{A diagram or worked example for the (i) \gls{ar} and (ii) \gls{me} case would help make this clearer and more convincing.}

\subsection{Supervised learning}\label{s:supervised_learning}
\subsubsection{\Acrlong{svm}}\label{s:support_vector_machine}
\gls{svm} is one of supervised machine learning algorithms \cite{noble_what_2006} that is used to analysis data through classification and regression in this paper. 
%\id{It is not clear what you are trying to suggest here}
%\mh{\done{Apart from \sref{support_vector_machine}, \sref{materials_and_methods} is largely background/theory \emph{not} materials and methods. I suggest you rename it to ``Background'', and rename \sref{experiments_and_material} as ``Materials and Methods''.}}
\mh{It is not clear that \sref{supervised_learning} belongs here.}

==> related_work.tex <==
\ts{Do I need to write related work? I feel it can be exist research about gait analysis or leg movement analysis if need. We could have a discussion.}
\mh{Yes, you need to draft a \nameref{s:related_work} section. This should cover any relevant related work (not only gait analysis, but also machine learning, information theory, wearables research). For an IEEE conference paper, typically \nameref{s:related_work} is very short, if present at all, so we may decide not to include it in the final conference submission. However, for a journal paper, and for your 9- and 18-month review reports, you need an extensive literature review. It is also helpful in organising your thoughts and ensuring your work really is filling a gap in the state of the art. So it is well worth drafting this now!}

There are numerous research papers focusing on human motion analysis based on sensor reading. However, the most of sensors are rigidly attached with the body. Very few studies use the signal collected from cloth-attached sensors in human motion analysis. 

One study \cite{jayasinghe_comparing_2019} investigates a comparison on activity classification performance across body-attached sensors and body-attached sensors with different cloth types (\eg slacks, pencil skirt and loose frock). The author collects acceleration signal during her multiple daily activities (walking, running, sitting, and riding a bus) on different segments of the body (waist, thigh, ankle). From this experiment’s result, it shows that it is promising to use cloth embedded sensor to classify different activities compared with body attached sensors. In addition, using signal collected from pencil skirt attached at waist has the better performance as it is tightly attached. While signal collected from loose frock attached at thigh has disappointed result because of fully randomly cloth movement. This research reveals cloth embedded sensor used for activity recognition has a good potential, particularly in daily real life.

Select suitable sensor configuration (e.g., sensor types and sensor position to provide more useful information in activity recognition is also a concern topic. This research \cite{gelenbe_sensor-activity_2013} uses mutual information to make an evaluation based on time-domain signal. This research places sensors on five positions (torso, right arm, left arm, right leg and left leg) and collect tri-axis signals by accelerometer, gyroscope and magnetometer. The author calculates the mutual information between activity classes and sensor measurement. High mutual information shows it provide more useful information in activity recognition. For signal directions, X-axis (perpendicular to the ground) has the highest mutual information at all sensor locations. In terms of sensor types, accelerometers provide more information than gyroscopes and magnetometers. Gyroscope is slightly higher than magnetometers. About sensor location, arm is the best sensor position, whereas the legs provide the lowest useful information.
